GazeMoDiff: Gaze-guided Diffusion Model for Stochastic Human Motion Prediction

Human motion prediction is important for many virtual and augmented reality (VR/AR) applications such as collision avoidance and realistic avatar generation. Existing methods have synthesised body motion only from observed past motion, despite the fact that human eye gaze is known to correlate strongly with body movements and is readily available in recent VR/AR headsets. We present GazeMoDiff - a novel gaze-guided denoising diffusion model to generate stochastic human motions. Our method first uses a gaze encoder and a motion encoder to extract the gaze and motion features respectively, then employs a graph attention network to fuse these features, and finally injects the gaze-motion features into a noise prediction network via a cross-attention mechanism to progressively generate multiple reasonable human motions in the future. Extensive experiments on the MoGaze and GIMO datasets demonstrate that our method outperforms the state-of-the-art methods by a large margin in terms of multi-modal final displacement error (17.3% on MoGaze and 13.3% on GIMO). We further conducted a human study (N=21) and validated that the motions generated by our method were perceived as both more precise and more realistic than those of prior methods. Taken together, these results reveal the significant information content available in eye gaze for stochastic human motion prediction as well as the effectiveness of our method in exploiting this information.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/conclusion.tex <==
\section{Conclusion}

In this work, we were the first to explore the effectiveness of eye gaze on generating multiple reasonable human motions in the future.
We proposed a novel gaze-guided diffusion model that fuses the gaze and motion features using a spatio-temporal graph attention network and then injects these features into a noise prediction network via a cross-attention mechanism to generate multiple reasonable human future motions. 
%first extracts spatio-temporal features from gaze and motion data and then uses these features to generate human future motions through a denoising diffusion process.
%Extensive experimental results 
%proposed a novel gaze-guided human motion diffusion framework to generate realistic motion predictions. Our approach involves an ST-GAT to capture the spatio-temporal correlations between eye gaze and human movements and extract cross-modal gaze-motion features. We then employed a cross-attention mechanism to inject this feature into the noise prediction network, which denoises the input Gaussian noise into diverse and realistic human full-body motions step by step. 
%\zhiming{The method description is too long. Only focus on your main contributions.} 
Extensive experiments demonstrated that our method outperforms the state-of-the-art methods by a large margin %in terms of prediction accuracy 
and a user study validated that our method can generate motions that are more precise and more realistic than prior methods.
%have shown significant improvements over several state-of-the-art methods in terms of accuracy.
%\zhiming{Add visualisation analysis and user study.}
%We further conducted a user study to evaluate the realism of the generated samples, which further confirmed that predictions from our method are perceived as more plausible.
As such, our work makes an important step towards generating more realistic human motions for virtual agents and guides future work on cross-modal human behaviour generation.
%establishes a foundation for gaze-guided stochastic human motion prediction and paved the way for future research in this crucial area of VR studies.

\section*{Acknowledgments}
This work was funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany's Excellence Strategy -- EXC 2075 -- 390740016.


==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/discussion.tex <==
\section{Discussion}
%\zhiming{Change the structure of this section to make it more compact.}
Our study marks a notable advancement in the emerging field of incorporating eye gaze cues for stochastic human motion prediction in VR/AR research. We have successfully demonstrated the effectiveness of our proposed method in generating multiple reasonable human motion predictions.

%\zhiming{Suggestions: 1. The effectiveness of eye gaze: refer to prior table/figure results of with and without eye gaze to show that eye gaze is useful for the task. Refer to the visualisation results and try to explain why eye gaze helps improve the performance 2. Performance of our method: use existing results to demonstrate that our method is more precise and more realistic. 3. Other important insights from the results, e.g. the results of adding gaze to other methods. Limitations: 1). we use complete observations while in real applications the observations may be incomplete (see the HOIMotion paper) 2). the number of datasets that contain both the eye gaze and body motions are limited limiting our evaluation 3). some limitations of general diffusion models, e.g. random generation/cannot be explicitly controlled. Future work: 1). explore more modalities 2). apply our model on real VR/AR applications 3). Improve the performance by using more powerful feature extraction and fusion methods.}

\textbf{Performance of our method.} Our method outperforms the state-of-the-art methods in terms of all metrics on both the MoGaze and GIMO datasets (See \autoref{tab:quantitative_result}). In addition, the visualisation results on both datasets showed that our method can generate multiple reasonable predictions with high precision while the state-of-the-art may produce erroneous or implausible predictions (\autoref{fig:teaser} and \autoref{fig:endpose_precise_case}).
%In contrast, HumanMAC yielded some implausible predictions. (See \autoref{fig:teaser} and \autoref{fig:endpose_precise_case}.) 
%And the differences between our method and HumanMAC are statistically significant. 
The results from a user study further confirmed that the predictions generated by our method were more realistic and more precise than that from prior method (\autoref{tab: user study}). These results demonstrate that our work have made a significant improvement in stochastic human motion prediction in terms of improving both precision and realism.

\textbf{The effectiveness of eye gaze for stochastic HMP.} To the best of our knowledge, our method is the first to introduce eye gaze in the stochastic HMP task to obtain a significant performance improvement.
Compared to the full model, the ablated version of not using eye gaze performed significantly worse on both datasets (\autoref{tab:quantitative_result}). It demonstrated that introducing the historical eye gaze as input can benefit the generation of more precise future motions. The visualisation example further demonstrated the effectiveness of incorporating eye gaze.
As shown in \autoref{fig:endpose_wo_gaze}, the observed motion showed a person turned to the right and then standing. The ground truth pose at future one second showed the person turning right again from a standstill. Our full model with eye gaze can predict this intention of turning right while the ablated version of not using eye gaze failed to recognise it and generated predictions that were all staying in place. 
We argue that the eye gaze implies the intention of future body movements. Therefore, our method can recognise more complex and precise intentions and make reasonable and precise predictions.

\textbf{The approach to introducing gaze into stochastic HMP.} Our method showed a significant improvement in the stochastic HMP task by adding eye gaze as input. A natural question is whether adding eye gaze as additional input to an existing method has an effect. In \autoref{sec:addinggaze} we explored existing diffusion-based methods with eye gaze as an additional joint input. The accuracy declined slightly on the GIMO dataset (\autoref{tab:quantitative_result_addinggaze}). Compared to the MoGaze dataset, the GIMO dataset contains more complex actions and motions, and the correlation between eye gaze and future action intent is much harder to mine. Therefore, simply adding eye gaze as an additional joint makes it difficult to model this complex correlation. Our method extracted the gaze and motion features via two encoders and fused them via GAT. Experimental results demonstrated the effectiveness of our gaze encoder, motion encoder, as well as the GAT (\autoref{tab: ablation_study}).

%We argue that the difference is derived from the datasets themselves. The MoGaze dataset only contains pick and place actions. Eye gaze is usually more closely and simply associated with the target movement. In contrast, the GIMO dataset contains more complex actions and motions, and the correlation between eye gaze and future action intent is much harder to mine. Therefore, simply adding eye gaze as an additional joint makes it difficult to model this complex correlation. Our method extracted the gaze and motion features via two encoders and fused them via GAT. Experimental results demonstrated the effectiveness of our gaze encoder, motion encoder, as well as the GAT (\autoref{tab: ablation_study}).

\textcolor{black}{\textbf{Diversity reduction due to eye gaze guidance.} As shown in \autoref{tab:quantitative_result}, our model reported obvious improvements in terms of all accuracy metrics. Intuitively, the diversity of predictions will decrease. To further explore whether and to what extent the diversity of our predictions were reduced, we used the average pairwise distance (APD), i.e. the average L2 distance between every pair of motion predictions, to measure the diversity. We observed that when ablating eye gaze from our model, the APD value increases from 15.572 to 15.799 on MoGaze and from 15.519 to 20.199 on GIMO. These results validate that while adding eye gaze can improve accuracy, it inevitably decreases the diversity of the motion predictions. %We argue that classifier-free guidance \cite{ho2022classifier} somewhat mitigates the decline.
}

%have demonstrated our approach to introducing gaze makes a significant improvement on the MoGaze and GIMO datasets.

%\textbf{Introducing eye gaze to stochastic HMP.} Introducing eye gaze as an additional modality allows the HMP model to generate more realistic and goal-directed poses\zhiming{goal-directed?}. 
%Eye gaze cues provide valuable information about a person's intentions and planned actions. In addition, the integration of eye gaze modality is highly practical. Modern VR headsets are equipped with built-in eye-tracking modules that can capture gaze data in real time. This means that gaze signals are readily available when using these devices, without the need for additional peripheral hardware.\zhiming{This does not need to be discussed again because it is clear in the motivation. More importantly, it is important to try to explain why eye gaze helps imporve the performance.} As presented in \autoref{tab:quantitative_result} and \autoref{tab: ablation_study}, gaze information indeed improves the accuracy of our model. 
%In addition, considering that gaze is not available in some cases, we tried to use head direction instead of gaze and achieved comparable results. This extends the use of the algorithm to VR devices without eye-tracking or when eye-tracking is impaired.
%\textbf{Introducing eye gaze to stochastic HMP.} 

%\zhiming{This could be put in the future work. In the discussion, before the limitations and future work parts, you should discuss existing results.}\textbf{Potential for extension to other modalities.} Our proposed approach, GazeMoDiff, has the potential to be extended to incorporate additional modalities beyond gaze. It serves as a multimodal human motion prediction framework, where various guidance information can be utilised to enhance the generation of reasonable motions. By incorporating modalities such as facial expressions, hand gestures, and physiological signals, the GazeMoDiff framework can be expanded to capture a more comprehensive range of cues for motion prediction. This multimodal approach can potentially lead to more contextually appropriate motion generation.

\textbf{Limitations.} 
First, only two public datasets contain both the eye gaze and body motions, limiting our evaluation's generalisability. In addition, existing datasets contain limited action categories, which make predictions that tend to be limited to a few number of actions and can not generalise to unseen actions.
%\zhiming{not clear why it is a limitation, not generalised to other actions?}
. Finally, our approach uses observed motions and eye gaze as input. However, the input data may be missing due to tracking errors in practical applications, which may limit the application of our method in real-world scenarios.

%We followed prior works\cite{chen2023humanmac,barquero2022belfusion,yuan2020dlow} to select APD as our diversity metric. But measuring different prediction distances in this way is too simple and crude, and it is susceptible to extreme values. As shown in \autoref{fig:endpose_faliure_case}, we observed cases where HumanMAC\cite{chen2023humanmac} and DLow\cite{yuan2020dlow} were prone to produce distorted poses. Movement trends were diverse measured by a high APD But extremely implausible. For accurate metrics, ADE and FDE, the error is the smallest one among all predictions. Image an extreme case in a model that generated 1 very accurate prediction and 99 distorted and unrealistic predictions. It would be evaluated as a state-of-the-art model in the APD-ADE-FDE metrics system. However, the most of predictions are useless and misleading for downstream analysis. That is also why we evaluated further through visualisation analysis and user study. Besides, 
%In our work, we predicted future motions by gaze and pose data. Gaze data is naturally available while pose needs to be captured by the wearable device. This may limit the application scenarios and be detrimental to the user experience. \zhiming{For HMP, generally we assume we have the poses.}
%\subsubsection{Trendy metrics}
%\subsubsection{Device dependency}

\textbf{Future work.}  Our proposed approach, GazeMoDiff, has the potential to be extended to incorporate additional modalities beyond eye gaze. It serves as a multi-modal human motion prediction framework, where various guidance information can be utilised to enhance the generation of reasonable motions. By incorporating modalities such as facial expressions, hand gestures, and physiological signals, the GazeMoDiff framework can be expanded to capture a more comprehensive range of cues for motion prediction. In addition, we are also looking forward to integrating our method with real VR/AR applications. Finally, as a diffusion-based prediction model, our method needs 100 DDIM sampling steps to denoise and obtain predictions, which limits to implementation into real-time scenarios. We will try some fast sampling methods~\cite{lu2022dpm,lu2022dpm++} to improve generation speed. %XXX \zhiming{add one more future work}%In our future research endeavours, we aim to explore the potential for extending our framework to incorporate a variety of modalities, such as emotional text, physical parameters, and scene information. Existing datasets only consist of partial modalities like MoGaze\cite{kratzer2020mogaze} (Motion and Gaze), GIMO \cite{zheng2022gimo} (Motion and Gaze) and EBEDB  (Gesture and Emotional label)\cite{volkova2014mpi}. It is worth exploring new datasets aggregating more modalities to enable more comprehensive multi-modal motion modeling and prediction. Additionally, to address the limitations associated with device dependency, we plan to develop a device-free approach. This approach would leverage different modalities, including gaze, motion, emotion, and scene information directly captured from video through learning-based estimation methods. By eliminating the need for users to wear specific devices or deploy complex sensors, this device-free method holds the potential to be applied in augmented reality or mixed reality scenarios, enhancing user experience and portability. 
%Furthermore, we recognise the need for improved metrics for stochastic human motion prediction. While metrics such as ADE, FDE, and APD have been widely used, there is room for further refinement and development of metrics that better capture the quality and usefulness of predicted motions. Enhancing the metrics will contribute to more accurate and comprehensive evaluations of human motion prediction methods.

==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/experiments.tex <==
\section{Experiments}

\subsection{Datasets}
\label{datasets}
%As the field of relating human movement to gaze to predict movement is just emerging\zhiming{just emerging? no, you should emphasise you are the first. Just say the datasets containing gaze and motion are limited.}, there are currently only a few public datasets available for experiments. 
Only a limited number of datasets contain synchronised recordings of both eye gaze and full-body human motion. 
We evaluated our method on two such public datasets, i.e. the MoGaze~\cite{kratzer2020mogaze} dataset for real-world setting and the GIMO~\cite{zheng2022gimo} dataset for AR setting.

\textbf{MoGaze.} The MoGaze dataset provides motion capture and eye-tracking data recorded simultaneously from 6 participants performing $pick$ and $place$ actions in an indoor environment.
It contains over 3 hours of body movement and eye gaze recordings captured at 30 Hz. The pose of the human body is expressed using the 3D coordinates %and Euler angles 
of 21 body joints while the eye gaze is represented as a direction vector. 
%Following prior work~\cite{chen2023humanmac,barquero2022belfusion,yuan2020dlow} on stochastic HMP, we represented the pose using only the 3D coordinates of each joint. The gaze vector was treated similarly to a virtual joint, with coordinates computed as the vector sum of the head joint coordinates and the gaze direction vector. This unified representation of both body pose and eye gaze solely in joint coordinate space allowed us to apply existing stochastic models to compare easily. 
%Without special notes, all $baselines + gaze$ donate to this implementation. 
Following common settings in stochastic human motion prediction~\cite{chen2023humanmac,barquero2022belfusion,yuan2020dlow}, we used recordings from $p1$, $p2$, $p4$, $p5$, and $p6$ for training and employed the data from $p7$ for testing.

\textbf{GIMO.} The GIMO dataset contains body motion and eye gaze data captured from 11 participants in various indoor AR environments.
%, as well as additional scene point cloud data captured for each manipulation task. However, as scene data may not be available in all VR scenarios, we only utilise the motion and gaze recordings for our experiments\zhiming{Don't mention the scene content here, otherwise it is misleading. Using scene content can be one of your future work.}. %covered in GIMO are richer than Mogaze
%\zhiming{Why do you emphasise this? No meaning to compare these two datasets.} 
%\reply{In quantitative results part, I argue some results may be caused by the richness of action types.}
The action categories include ${sitting}$ or ${laying}$ ${on}$ ${objects}$, ${touching}$, ${holding}$, ${reaching}$ ${to}$ ${objects}$, $opening$, $pushing$, $transferring$, $throwing$, $swapping$ $objects$, etc. 
%The skeletal model consists of 23 body joints. 
We represented the body pose in the GIMO dataset using the 3D coordinates of $23$ body joints and denoted the eye gaze using a direction vector.
In the evaluation process, we followed the official dataset splits provided in GIMO~\cite{zheng2022gimo}. 
The training set comprises motion and eye gaze recordings from 12 scenes, while the test set contains data from 14 scenes, including 12 known environments and 2 new, unseen environments. 
This evaluation protocol allows the assessment of generalisation capabilities to new scenes.

\subsection{Evaluation Metrics}
To evaluate the performance of our model, we employed four commonly used metrics following prior works on stochastic HMP~\cite{yuan2020dlow,saadatnejad2023generic,chen2023humanmac}:% \zhiming{cite the icra paper that uses the four metrics}

%\textbf{Average Pairwise Distance (APD)} measures diversity as the average L2 distance between all motion examples generated by the model. Higher APD indicates more diverse predictions.

\begin{itemize}
    \item Average displacement error (ADE): ADE measures the average $l_2$ distance between the ground truth and the predicted motions over the whole future sequence. The lower the ADE, the more precise the prediction.
    
    \item Final displacement error (FDE): FDE calculates the $l_2$ distance between the ground truth and the predicted future motions at the final timestep.
    The lower the FDE, the more precise the prediction at the final timestep.
    
    \item Multi-modal average displacement error (MMADE): MMADE is designed to handle the multi-modal nature of the predictions in the task of stochastic HMP. It takes into account the fact that there can be multiple reasonable ground truth sequences for a given input. The multiple ground truth is obtained from the future motions of similar observed sequences (Sequences with $l_2$ distance below a given threshold are treated as similar sequences). MMADE is the mean value of the ADE calculated using the predictions and the multiple ground truth.
    %\zhiming{It is still unclear how it is calculated. It is using the mean error of multiple GT or the best error? Also, how 'clustering similar past motions' is performed is unclear.} 
    The lower the MMADE, the better the ability to generate multiple reasonable predictions.
    
    \item Multi-modal final displacement error (MMFDE): MMFDE is calculated in a similar way as MMADE. The difference is that MMADE calculates the average $l_2$ distance over all future timesteps while MMFDE measures the $l_2$ distance only at the final timestep.
    The lower the MMFDE, the better the ability to generate multiple reasonable predictions at the final timestep.
\end{itemize}

%\textcolor{black}{Note that all evaluation metrics are in meters.}
%\textbf{Average Displacement Error (ADE)} and \textbf{Final Displacement Error (FDE)} measure accuracy. ADE is the average L2 distance between ground truth and predicted motions over the whole future sequence. FDE is the L2 distance at the final timestep. Lower ADE and FDE indicate more accurate predictions.

%\textbf{Multi-Modal Average Displacement Error (MMADE)} and \textbf{Multi-Modal Final Displacement Error (MMFDE)} are are metrics specifically designed to handle the multi-modal nature of predictions in stochastic HMP tasks. These metrics take into account the fact that there can be multiple plausible ground truth sequences for a given input. The multiple plausible ground truth sequences are obtained by clustering similar past motions. Lower MMADE and MMFDE indicate a better ability to generate different plausible predictions.

\subsection{Baselines}
We compared our method with the following state-of-the-art methods in stochastic human motion prediction: %and their variants\zhiming{variants sound weird. You can say for fair comparison, you add gaze to SOTA. BTW, why no gaze for DLow and CVAE? You need a motivation for adding gaze only to these two.}:
\begin{itemize}    
    \item \textit{DLow}~\cite{yuan2020dlow}: \textit{DLow} is a latent flow-based model to generate multiple future motions via diversity-promoting sampling and loss.
    
    \item \textit{CVAE}~\cite{yuan2020dlow}: \textit{CVAE} is a conditional variational autoencoder utilised in DLow~\cite{yuan2020dlow} as a pre-trained generative model which can also forecast stochastic future motions.
    
    \item \textit{BeLFusion}\cite{barquero2022belfusion}: \textit{BeLFusion} is a latent diffusion-based model to predict reasonable motions based on %benefited from 
    disentangling the behavioural representation from past motions.%\zhiming{past poses and motions?}
    
    \item \textit{HumanMAC}\cite{chen2023humanmac}: \textit{HumanMac} is a diffusion-based stochastic HMP model with a DCT completion fashion in the inference.
    %n end-to-end single-loss stochastic HMP model with a DCT completion fashion in the inference. 
    %\item \textit{BeLFusion+gaze}: We introduce gaze into \textit{BeLFusion} by regarding gaze as a virtual joint as described in \autoref{datasets}. 
    %\item \textit{HumanMac+gaze}: We introduce gaze into \textit{HumanMac} in the same way.
\end{itemize}

\subsection{Implementation Details}

We set the observation and prediction time windows to 0.5 seconds (15 frames) and 2 seconds (60 frames) respectively for both the MoGaze and GIMO datasets, following common practice in stochastic human motion prediction~\cite{chen2023humanmac,barquero2022belfusion,yuan2020dlow}.
%As baselines are not evaluated on MoGaze and GIMO, We need to train them from scratch. 
For a fair comparison, we retrained all the baseline methods from scratch using their default training parameters. %and settings were kept at their default values
We trained all the modules in our method in an end-to-end manner for 300 epochs using Adam optimiser\cite{kingma2014adam} with an initial learning rate of 0.0003 and a batch size of 32.
The learning rate was decayed at 75, 150, 225, 275 epochs, respectively, with a multiplicative factor of 0.9.
%The multi-step learning rate scheduler was set to $\gamma = 0.9$ in our model and the learning rate was decayed at 75, 150, 225, 275 epochs, respectively. %\zhiming{At which steps you use the scheduler?}.
%For both datasets, we applied the same training and hyperparameter settings, we jointly trained the gaze-motion fusion network and the noise prediction network using 
We applied a standard diffusion process as proposed by~\cite{song2020denoising} that degraded 1500 steps in the training and sampled 100 steps in the inference. 
We selected the Cosine noise scheduler~\cite{nichol2021improved} in the diffusion 
%\zhiming{what is the Cosine scheduler used for}
following HumanMAC~\cite{chen2023humanmac}. 
The multi-modal ground truth %\zhiming{which clustering method you used to obtain the multi-modal ground truth} 
threshold was set to 0.4 following previous work~\cite{barquero2022belfusion}.
%\zhiming{The parameters of the network can be put in the places you introduced them. Here you only introduce the training settings.} 
All experiments were conducted in an Nvidia TITAN X GPU with 12GB memory using the PyTorch 1.7.1 framework.

\subsection{Quantitative Results}

\begin{table*}[ht]
  \caption{Comparison of our method with the state-of-the-art methods on both MoGaze~\cite{kratzer2020mogaze} and GIMO~\cite{zheng2022gimo} (unit: meters). The best results are in bold while the second best are underlined.} 
  %\zhiming{Separate the two +gaze methods using a line to stress that they are not existing methods.}}
  %\zhiming{Can you use a vertical line to separate the two results?}}
  \label{tab:quantitative_result}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	l%
	*{4}{c}
        |c
        *{3}{c}%
	%
	}
  \toprule
  & \multicolumn{4}{c}{Results on MoGaze~\cite{kratzer2020mogaze}} & \multicolumn{4}{c}{Results on GIMO~\cite{zheng2022gimo}} \\
  \midrule
    %& APD~$\uparrow$ &  ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$ & APD ~$\uparrow$&  ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$\\
    &  ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$ &ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$\\
  \midrule
    %\textit{CVAE}\cite{yuan2020dlow}& \underline {17.900} &  1.070 &   1.644 & 1.091 & 1.667 &  \underline{20.297}&  1.292 &   2.059 & 1.294 & 2.054\\
    \textit{CVAE}\cite{yuan2020dlow} &  1.070 &   1.644 & 1.091 & 1.667 &    1.292 &   2.059 & 1.294 & 2.054\\
    
    %\textit{DLow}\cite{yuan2020dlow}& \textbf{22.277} &  0.807 &   1.261 & 0.840 & 1.274 &  \textbf{24.538}&  1.084 &   1.688 & 1.090 & 1.687\\
    \textit{DLow}\cite{yuan2020dlow} &  0.807 &   1.261 & 0.840 & 1.274 &  1.084 &   1.688 & 1.090 & 1.687\\
     
     %\textit{BeLFusion}\cite{barquero2022belfusion}& 17.099 &  0.899 &   1.306 & 0.908 & 1.313 &  17.959&  0.840 &   1.220 & 0.845 & 1.221\\
     \textit{BeLFusion}\cite{barquero2022belfusion} &  0.899 &   1.306 & 0.908 & 1.313 &  0.840 &   1.220 & 0.845 & 1.221\\
     
       %\textit{HumanMAC} \cite{chen2023humanmac}& 11.867 &  0.732 &   1.089 & 0.779 & 1.144 & 15.040 &  0.815 &   1.121 & 0.821 & 1.118\\
       \textit{HumanMAC} \cite{chen2023humanmac} &  0.732 &   1.089 & 0.779 & 1.144  &  0.815 &   1.121 & 0.821 & 1.118\\
      
        %\textit{BeLFusion+gaze }& 15.711 &  \underline{0.654} &   1.018 & \underline{0.659} & 1.012 & 15.237 &  0.858 &   1.226 & 0.861 & 1.221\\
        %\textit{HumanMAC+gaze }& 13.513 &  \underline{0.654} &   \underline{0.965} & 0.679 & \underline{0.980} & 15.682 &  0.850 &  1.135 & 0.852 & \underline{1.137}\\
        \midrule
        %$Ours_{head}$ & 10.959 &  \underline{0.648} &  \underline{1.003} & \underline{0.678} & \underline{1.018} & 15.574 &  \underline{0.776} &  \underline{1.058} & \underline{0.782} & \underline{1.064}\\
        %\textit{$Ours_{w/o \ gaze}$}& 15.799 &  0.664 &  0.982 & 0.696 & 0.996& 15.519 &  \textbf{0.729} & \textbf{ 0.974} & \textbf{0.732} & \textbf{0.969}\\
        \textit{$Ours_{w/o \ gaze}$} &  \underline{0.664} &  0.982 & 0.696 & 0.996&  0.812 & 1.120 & 0.818 & 1.116\\
        \textcolor{black}{\textit{$Ours_{head}$}}&  \textcolor{black}{0.669} &  \textcolor{black}{\underline{0.971}}& \textcolor{black}{\underline{0.678}} & \textcolor{black}{\underline{0.974}} &  \textcolor{black}{\underline{0.734}} & \textcolor{black}{\underline{0.979}} & \textcolor{black}{\underline{0.737}} & \textcolor{black}{\underline{0.975}}\\
         %\textit{Our}& 15.572 &  \textbf{0.638} &  \textbf{ 0.939} & \textbf{0.649} & \textbf{0.946 }& 15.519 &  \textbf{0.729} & \textbf{ 0.974} & \textbf{0.732} & \textbf{0.969}\\

         
         \textit{Ours} &  \textbf{0.638} &  \textbf{ 0.939} & \textbf{0.649} & \textbf{0.946 } &  \textbf{0.729} & \textbf{ 0.974} & \textbf{0.732} & \textbf{0.969}\\
  
  \bottomrule
  \end{tabu}%
\end{table*}

The quantitative results on the MoGaze~\cite{kratzer2020mogaze} and GIMO~\cite{zheng2022gimo} datasets are shown in \autoref{tab:quantitative_result}.
Overall, our model outperforms the state-of-the-art methods on all metrics. 
%while maintaining reasonable prediction diversity.

\textbf{Results on MoGaze.} As shown in \autoref{tab:quantitative_result}, our model achieves the lowest ADE, FDE, MMADE and MMFDE compared to prior methods, substantially surpassing the best state-of-the-art HumanMAC~\cite{chen2023humanmac}. For average displacement error, our method achieves an improvement of 12.8\% (0.638 $vs.$ 0.732) over HumanMAC\cite{chen2023humanmac}. On final displacement error, our method obtains a 13.7\% performance gain (0.939 $vs.$ 1.089). 
%These significant improvements demonstrate our method fully extracted and fused the informative eye gaze and motion sequence.\zhiming{not strong evidence}
On multi-modal accuracy metrics, our method improves the MMADE performance by 16.7\% (0.649 $vs.$ 0.779) and the MMFDE performance by 17.3\% (0.946 $vs.$ 1.144). The greater gains on the multi-modal metrics reveal that our model is more capable of generating multiple reasonable predictions aligned with the stochasticity of human nature.
%producing multimodal predictions aligned with the stochasticity of human nature.
%A Wilcoxon signed-rank test\cite{wilcoxon1992individual} indicates a statistically significant ADE difference ($p<0.01$) between our method and HumanMAC. 
%\zhiming{This test should be done for all the metrics. see following sentence}
We further conducted a Wilcoxon signed-rank test to compare our method and the state-of-the-art and the results demonstrate that the differences between our method and the state-of-the-art method are statistically significant ($p<0.01$).
%Although diversity reduces due to gaze-guided predictions, compared to DLow with the highest APD, our method outperforms by 22.92\%, 26.80\%, 30.40\% and 27.00\% in terms of ADE, FDE, MMADE and MMFDE. It implies the predictions of DLow are not plausible so the diversity is meaningless somehow. 
In addition, we also presented the performance of our method without using eye gaze in Table~\ref{tab:quantitative_result}. Compared to our method, the ablated version of not using eye gaze presents lower accuracy in terms of ADE, FDE, MMADE and MMFDE, demonstrating the effectiveness of eye gaze information for stochastic human motion prediction.
It is also notable that our method without using eye gaze still outperforms the state-of-the-art methods, achieving an improvement of 9.8\% on MMADE and 12.9\% %\zhiming{add the values}
on MMFDE.
%$Ours_{w/o \ gaze}$ outperforms other baselines without gaze, as presented in . 
These results underscore the superiority of our model architecture. Considering that eye gaze is not always available, we further present a novel variant that replaces gaze with head direction. We can see from Table~\ref{tab:quantitative_result} that although this variant is not as good as our full model, it outperforms the variant without gaze. These results demonstrate that head direction can be a reliable alternative when gaze is not available.
%finding underscores the superiority of our proposed framework, whether or not gaze information is involved.

\textbf{Results on GIMO.} As shown in \autoref{tab:quantitative_result}, our method outperforms the state-of-the-art methods in all the metrics.
%is still superior among the state-of-the-art methods in all accuracy metrics. 
Specifically, compared to the state-of-the-art method HumanMAC, our method achieves an improvement of 10.5\% (0.815 to 0.729) in ADE as well as an improvement of 13.1\% (1.121 to 0.974) in FDE.
%Our model lowers ADE by 10.5\% compared to HumanMAC (0.815 to 0.729) and reduces FDE by 13.1\% (1.121 to 0.974). 
On multi-modal accuracy metrics, our method obtains an improvement of 10.8\% in MMADE and 13.3\% in MMFDE, respectively.
%we attain 10.8\% and 13.3\% improvements in MMADE and MMFDE respectively. 
The results from a Wilcoxon signed-rank test validate that the differences between our method and the state-of-the-art method are statistically significant ($p<0.01$).
We also find that our method significantly outperforms the ablated version of not using eye gaze, revealing the importance of eye gaze for generating stochastic human motions. \textcolor{black}{The results of $Ours_{head}$ on GIMO also validate that eye gaze performs better than head orientation in terms of human motion prediction and revealed that head orientation can be used as a proxy to gaze when gaze is not available.}
%compared to our method, the ablated version of not using eye gaze 
%Compared to our method, the .
%\textit{GazeMoDiff}, the variant without gaze presents lower accuracy in terms of all metrics on GIMO, which also reveals that eye gaze is informative for precise motion prediction. 
%This demonstrates the strong generalisation ability \reply{Question: I am not sure if it is precise} of our approach to a new dataset.\zhiming{This usually means you train on one dataset and test on another} 
%A Wilcoxon signed-rank test again showed a significant ADE difference ($p<0.01$) versus HumanMAC. 

%DLow also shows the highest APD values but particularly low accuracy on this dataset. Our method is superior to DLow by 30.9\%, 39.51\%, 30.83\% and 39.18\% in terms of ADE, FDE, MMADE and MMFDE, respectively. Additionally, previous work\cite{tevet2022human} pointed out that methods with high diversity metrics but low accuracy may suffer failure predictions. We will further discuss this phenomenon in \autoref{visulisationAn}. 

%Compared to gaze-agnostic methods CVAE and DLow, we surpass them by 8.02\%-30.52\% in MMADE, and 12.23\%-38.64\% in MMFDE.

%This clearly validates the importance of leveraging gaze cues for motion prediction.
%\zhiming{You can give the results on MoGaze and GIMO respectively. Give the percentages of improvements as you did in the abstract and intro. Disucss the results on each dataset and go into different metrics. This is the most important result part and should be explained in detail.}

%From the perspective of datasets, the larger performance gap of GazeMoDiff compared to non-gaze methods on Mogaze can be attributed to the stronger correlation between eye movements and body motion inherent in the dataset.\zhiming{I am not convinced by your explanation here because you don't have strong evidence for this.} Mogaze primarily contains picking and placing actions, which intimately rely on visual cues from gaze to direct the hands to targeted objects. These object manipulation tasks make the correlations between future pose trajectories and eye movement patterns easier to capture. Thus, the variants adding gaze of BeLFusion and HumanMAC are also comparable.

%In contrast, the activities in GIMO like laying, sitting etc. involve full-body motions that are not always as strictly coupled to moment-to-moment changes in gaze direction\zhiming{You do not have evidence for this.}. Thus simply introducing gaze as a joint doesn't work on BeLFusion and HumanMAC. Our spatiotemporal GAT is designed to capture this complex correlation and extract high-level intent information from this correlation. Therefore, our model is superior to baseline variants with added gaze.
%It demonstrates the effectiveness of introducing gaze and reveals our framework, especially the spatio-temporal GAT and cross-attention mechanism can fully integrate gaze with poses to generate more realistic motions.

%Compared to baselines without gaze input, especially, our method substantially reduces ADE and FDE on both datasets by a large margin. This is because gaze direction provides crucial cues for future motions, and our spatiotemporal GAT within the diffusion model can effectively leverage this information to constrain predictions. 

%Some baselines like DLow with the highest diversity suffer very low accuracy (), which implies their predictions are not plausible and there would be some failure predictions.

%We also introduce simply into HumanMAC\cite{chen2023humanmac} and BeLFusion\cite{barquero2022belfusion}. These variants improve accuracy on MoGaze\cite{kratzer2020mogaze} while their accuracy does not change significantly on GIMO\cite{zheng2022gimo}. It demonstrates that introducing the gaze simply doesn't always improve the accuracy. This demonstrates that simply adding gaze does not always yield benefits - the network must be carefully designed to properly capture spatiotemporal relationships and fully utilise gaze for guidance. 
\subsection{Visualisation Analysis}
\label{visulisationAn}

%\begin{figure*}[ht]
%  \centering
%\includegraphics[width=\textwidth]{figs/poses_mogaze.pdf}

%\caption{Qualitative results about the orientation of predictions. The first two columns denote the first frame and last frame of observation. GT means the ground truth of 1s later. The rest of the 10 columns are predicted poses. \hl{The ground truth poses show a continued right turn of about 90 degrees further. Predictions from HumanMAC and DLow generally fail to anticipate the full turn, while our gaze-guided method is better able to recognise the intention to keep turning right attributed to gaze information.}}%\zhiming{What's the main conclusion from the visualisations?} 
%\label{fig:endpose_direction}
%\end{figure*}

We visualised the multiple predicted poses at the time point of the future one second.
We compared our method with %the best diversity baseline, DLow\cite{yuan2020dlow}, and 
the state-of-the-art method HumanMAC~\cite{chen2023humanmac}.
%\zhiming{Why do you only compare with these two methods rather than all the baselines? You need a strong motivation for this. This is also why you need to separate the to +gaze methods. Otherwise, people would argue why not compare with them. Here the motivation could be one is best in accuracy and the other is best in diversity.}. 
For each method, we randomly generated 10 predictions for comparison.

%\zhiming{Use a name for each of the following three paragraphs to emphasise which parts you are analysing.}
\textbf{Visualisation results on the MoGaze dataset.} We illustrated a representative visualisation from the MoGaze dataset \cite{zheng2022gimo} in \autoref{fig:endpose_precise_case}. The observed motion sequence involves a turn to the right, and the ground truth pose shows that at the future one second, this person continues the turn by about 100 degrees further to the right. We can observe that predictions of HumanMAC\cite{chen2023humanmac} % and DLow\cite{yuan2020dlow} 
generally continue walking in the same forward direction as the observed last frame, failing to anticipate the full turning trajectory.  The best prediction generated by HumanMAC~\cite{chen2023humanmac} (labelled in green) also differs from the ground truth. In contrast, our method can recognise that the person intends to keep turning right. As a result, the best prediction from our method is precisely facing the true direction of the ground truth and other predictions generally align with the ground truth. 
%Due to the inherent uncertainty in predicting future speed, the body orientations of our predictions differ slightly from each other, reflecting the range of plausible orientation angles given the observed turning motion. 
In addition, we can see that the poses generated by our method are physically plausible without any angle distortions or strange limb lengths.

%\textbf{Extreme case.} \autoref{fig:endpose_extremecase} illustrates an extreme case where the observed motion in the first 0.5s is walking straight ahead, while the ground truth pose 1s in the future involves a turn to the left. For baseline methods like HumanMAC and DLow that rely solely on historical pose information, there is no cue regarding the impending turn. As a result, all of their predictions continue facing the original forward direction. In contrast, our method leverages historical gaze directions which can provide hints about intended future actions. As shown boxed in red in \autoref{fig:endpose_extremecase}, one of our predictions is able to accurately anticipate the left turn, even in this scenario with minimal historical motion context. While only a single prediction succeeded in this extreme case of lacking pose cues, such predictions that can foresee abrupt changes are still very valuable, especially for safety-critical applications involving collision avoidance.


\textbf{Visualisation results on the GIMO dataset.} We also illustrated a typical visualisation from the GIMO dataset~\cite{zheng2022gimo}. As depicted in \autoref{fig:teaser}, predictions from our method are more similar to the ground truth. Furthermore, all predictions from our method are generally realistic. In contrast, HumanMAC yielded predictions that include some implausible cases (boxed in red). These results demonstrate that our method can generate more reasonable motion predictions than the state-of-the-art.

%It revealed that our methods can learn the topological relationship between joints and keep it when predicting.%Corresponding with prior findings\cite{chen2023humanmac}, we argued that some baselines like DLow achieved high APD but suffered from implausible cases. Despite the high APD calculated for these implausible prediction samples, they are meaningless and misleading for downstream tasks in fact. In contrast, predictions from our approach look natural with diversity.

\textbf{Visualisation results of not using eye gaze.} To further evaluate the effectiveness of eye gaze for stochastic human motion prediction, we showed a visualisation example to compare our method with the ablated version of not using eye gaze.
As shown in \autoref{fig:endpose_wo_gaze}, the observed motions showed a person turning to the right and then standing still. 
Our method was able to predict that the person would continue going right in the future while the ablated version of not using eye gaze failed to recognise this intention and stayed in place.
These results demonstrate that eye gaze signals provide information on human intention and can help improve the performance of stochastic human motion prediction methods.

%It demonstrated that eye gaze contains information about intentions, and combining it with observed movements can guide more accurate predictions of future motions.

More visualisation results are provided in the supplementary material.

\begin{figure*}[ht]
  \centering
    \includegraphics[width=\textwidth]{figs/poses_precise_case.pdf}
\caption{Ground truth (GT) human pose at future one second and multiple pose predictions generated by different methods on the MoGaze dataset~\cite{kratzer2020mogaze} with the best prediction (lowest $l_2$ distance to GT) boxed in green.
Our method can generate motions that are closer to the ground truth than the state-of-the-art method HumanMAC~\cite{chen2023humanmac}.}
%\zhiming{What's the main conclusion from the visualisations?}}
\label{fig:endpose_precise_case}
\end{figure*}

\begin{figure*}[ht]
  \centering
    \includegraphics[width=\textwidth]{figs/poses_precise_case_wogaze.pdf}
\caption{Ground truth (GT) human pose at future one second and multiple pose predictions generated by different methods on the MoGaze dataset~\cite{kratzer2020mogaze} with the best prediction (lowest $l_2$ distance to GT) boxed in green. Our method using eye gaze can generate motions that are closer to the ground truth than the ablated version of not using eye gaze.}
%\zhiming{What's the main conclusion from the visualisations?}}
\label{fig:endpose_wo_gaze}
\end{figure*}

\subsection{Adding Eye Gaze to Prior Methods}\label{sec:addinggaze}
%\zhiming{put the results of baseline+gaze here.}

To further evaluate our method's effectiveness for extracting and fusing gaze and motion features, we compared our methods with prior methods' variants that add eye gaze as input. The results on MoGaze and GIMO are shown in \autoref{tab:quantitative_result_addinggaze}, where $Hum_{gaze}$ and $BeL_{gaze}$ denotes the variants of HumanMAC and BeLFusion that add eye gaze as an extra input joint. Overall, our approach outperforms both BeLFusion and HumanMAC which incorporate eye gaze information in terms of all metrics, demonstrating our method's superiority in exploiting eye gaze information.
Additionally, compared to the performance of original HumanMAC and BeLFusion shown in \autoref{tab:quantitative_result}, all the metrics improve on the MoGaze dataset while getting worse slightly on the GIMO dataset.
It demonstrates that simply adding eye gaze as a new joint to an existing method does not always have a positive effect. 
Instead, the internal features of the eye gaze and its synergistic correlations with other human joint nodes need to be considered. 
Our approach outperforms the state-of-the-art methods significantly by introducing novel feature extraction and fusion modules for gazes and motions and using the fused features to guide future motion generation. %through a denoising network based on the cross-attention mechanism. 

\begin{table}[ht]
  \caption{Comparison of our method with baselines that add eye gaze as input on both MoGaze~\cite{kratzer2020mogaze} and GIMO~\cite{zheng2022gimo} (unit: meters). The best results are in bold while the second best are underlined.} 
  %\zhiming{Separate the two +gaze methods using a line to stress that they are not existing methods.}}
  %\zhiming{Can you use a vertical line to separate the two results?}}
  \label{tab:quantitative_result_addinggaze}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	*{6}{l}%
	%
	}


  \toprule
    Dataset & Method&  ADE &   FDE & MMADE & MMFDE \\
  \midrule
    %\textit{HumanMAC+gaze }& 13.513 &  \underline{0.654} &   \underline{0.965} & 0.679 & \underline{0.980} & 15.682 &  0.850 &  1.135 & 0.852 & \underline{1.137}\\
    %\textit{BeLFusion+gaze }& 15.711 &  \underline{0.654} &   1.018 & \underline{0.659} & 1.012 & 15.237 &  0.858 &   1.226 & 0.861 & 1.221\\
%\textit{Our} &  \textbf{0.638} &  \textbf{ 0.939} & \textbf{0.649} & \textbf{0.946 } &  \textbf{0.729} & \textbf{ 0.974} & \textbf{0.732} & \textbf{0.969}\\
    \multirow{3}{*}{MoGaze}
   &$Hum_{gaze}$ &\underline{0.654} &   \underline{0.965} & 0.679 & \underline{0.980} \\ 
   &$BeL_{gaze}$ &\underline{0.654} &   1.018 & \underline{0.659} & 1.012 \\
   &\textit{Ours} &\textbf{0.638} &  \textbf{ 0.939} & \textbf{0.649} &\textbf{0.946 } \\
   \midrule
   \multirow{3}{*}{GIMO}
   & $Hum_{gaze}$ &\underline{0.850} &   \underline{1.135} & 0.852 & \underline{1.137} \\ 
   &$BeL_{gaze}$ &  \underline{0.858} &   1.126 & \underline{0.861} & 1.221 \\
   &\textit{Ours} &\textbf{0.729} &  \textbf{ 0.974} & \textbf{0.732} &\textbf{0.969 } \\
   %$Ours_{w/o \ gaze}$&15.772  &0.694   &1.016   &0.721  &1.031  \\
   %$Ours_{w/o \ cfg}$&12.478  &0.677   &1.048   &0.710  &1.063  \\
   %\midrule
   %$BeLFusion_{g}$& \textbf{15.711} & 0.654 &   1.018 & 0.659 & 1.012 \\
   %$HumanMAC_{g}$& 13.783 &  0.650 &   0.959 & 0.660 & 0.967 \\
  \bottomrule
  \end{tabu}%
\end{table}

\subsection{Ablation Study}
We conducted an ablation study to comprehensively analyse the individual contributions of various modules within our framework. %and evaluate the specific impact of incorporating gaze information.
We thoroughly assessed the performance of our model by comparing it to variants that exclude specific modules:
\begin{itemize}
    \item  $Ours_{w/o \ gat}$ : Without spatio-temporal graph attention network.
    \item $Ours_{w/o \ CA}$ : Without cross attention in the noise predicting network.
    %\item $Ours_{w/o \ gaze}$ : Without gaze 
    \item $Ours_{w/o \ GE}$ : Without gaze encoder.
    \item $Ours_{w/o \ ME}$ : Without motion encoder.
    %\item $Ours_{w/o \ cfg}$ : Without classifier-free guidance
    %\item  $Ours_{head}$: Replacing gaze with head direction
\end{itemize}

%Furthermore, we also compared our method to two diffusion baselines that incorporate gaze guidance.
%\begin{itemize}
%    \item  $BeLFusion_{g}$: We introduce gaze into \textit{BeLFusion} by regarding gaze as a virtual joint as described in \autoref{datasets}. 
 %   \item  $HumanMAC_{g}$: We introduce gaze into \textit{HumanMac} in the same way.
%\end{itemize}

%\zhiming{Make the best results in bold.}
As we can see from \autoref{tab: ablation_study}, our model outperforms all the ablated versions. %and baseline methods with gaze. 
It reveals that each module within our framework significantly contributes to the generation of stochastic human future motions.
%There are three notable findings worth discussing. 
%1) Compared to \textit{GazeMoDiff}, the variant without gaze presents obviously lower accuracy in terms of both ADE and FDE, which demonstrates gaze information is effective. 

%2) Despite the variant without gaze not surpassing the performance \textit{GazeMoDiff}, it notably outperforms other baselines without gaze, as presented in Table \ref{tab:quantitative_result}. This finding underscores the superiority of our proposed framework, whether or not gaze information is involved. 
%3) Our approach outperforms both BeLFusion and HumanMAC which incorporate gaze information in terms of all accuracy metrics, showing the effective utilisation of gaze information to enhance overall performance.
%3) Considering that in some scenarios where gaze is unavailable, we present a novel variant that replaces gaze with head direction. Although the accuracy metrics of this variant can not reach \textit{GazeMoDiff}, it can generate more accurate results than the variants without gaze. Thus head direction can be a reliable alternative when gaze is unavailable. 
%
\begin{table}[H]
  \caption{Ablation study on MoGaze\cite{kratzer2020mogaze}. The best results are in bold.}
  %\zhiming{You can only use the two +gaze versions here to show that your overall structure is better. +gaze versions should not appear in Table 1, otherwise they become the best baselines that you need to compare in your user study. Maybe it is better to remove them, otherwise people would expect you to compare with them in user study.}}
  \label{tab: ablation_study}
  \scriptsize%
    \centering%
\resizebox{0.47\textwidth}{!}{
  \begin{tabu}{%
	l%
	*{4}{c}%
	%
	}


  \toprule
    %& APD ~$\uparrow$&  ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$ \\
    &  ADE~$\downarrow$ &   FDE~$\downarrow$ & MMADE~$\downarrow$ & MMFDE~$\downarrow$ \\
  \midrule
    %\textit{HumanMAC+gaze }& 13.513 &  \underline{0.654} &   \underline{0.965} & 0.679 & \underline{0.980} & 15.682 &  0.850 &  1.135 & 0.852 & \underline{1.137}\\
  
   
   %$Ours_{w/o \ gat}$ &12.031&	0.655&	0.990&	0.663&	0.993 \\ 
   $Ours_{w/o \ gat}$ &	0.655&	0.990&	0.663&	0.993 \\ 
   %$Ours_{w/o \ CA}$ &11.809&	0.697&	1.001&	0.709&	1.000  \\
   $Ours_{w/o \ CA}$ &	0.697&	1.001&	0.709&	1.000  \\
   %$Ours_{w/o \ GE}$ &16.224&	0.655&	0.946&	0.665&	0.946 \\
   $Ours_{w/o \ GE}$ &	0.655&	0.946&	0.665&	\textbf{0.946} \\
   %$Ours_{w/o \ ME}$ &12.759&	0.642&	0.976&	0.654&	0.985 \\
   $Ours_{w/o \ ME}$ &	0.642&	0.976&	0.654&	0.985 \\
   %$Ours_{w/o \ gaze}$&15.772  &0.694   &1.016   &0.721  &1.031  \\
   %$Ours_{w/o \ cfg}$&12.478  &0.677   &1.048   &0.710  &1.063  \\
   %\midrule
   %$BeLFusion_{g}$& \textbf{15.711} & 0.654 &   1.018 & 0.659 & 1.012 \\
   %$HumanMAC_{g}$& 13.783 &  0.650 &   0.959 & 0.660 & 0.967 \\
   \midrule
   %$Ours_{head}$& 10.959& 0.648  &  1.003 & 0.678 &  1.018\\
   %$Ours$ &15.572  & \textbf{ 0.638} &  \textbf{0.939} & \textbf{0.649 }& \textbf{0.946} \\  
   $Ours$  & \textbf{ 0.638} &  \textbf{0.939} & \textbf{0.649 }& \textbf{0.946} \\
  \bottomrule
  \end{tabu}%
  }
\end{table}
%\begin{table}[H]
%  \caption{Ablation study on GIMO\cite{zheng2022gimo}}
%  \label{tab: ablation_study}
%  \scriptsize%

%	\centering%
%  \begin{tabu}{%
%	l%
%	*{5}{c}%
	%
%	}


%  \toprule
%    & APD &  ADE &   FDE & MMADE & MMFDE \\
%  \midrule
%   $Ours_{w/o \ gat}$ &13.222&	0.813&	1.111&	0.827&	1.123 \\ 
%   $Ours_{w/o \ CA}$ &19.395&	0.923&	1.185&	0.927&	1.189  \\
%   $Ours_{w/o \ gaze}$&16.540  &0.779   &1.078   &0.788  &1.079  \\
%   $Ours_{head}$& &   &   &  &  \\
%   $Ours$ &14.916 &  0.752 &  1.021 & 0.761 & 1.032 \\
     
  
%  \bottomrule
%  \end{tabu}%
%\end{table}



==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/introduction.tex <==
\firstsection{Introduction}
\maketitle

Generating realistic human body movements is a key research challenge in the area of virtual and augmented reality (VR/AR) and is the basis for safe, smooth, and immersive human-environment~\cite{david2021towards, sun2018towards} and human-human interactions~\cite{kim2017activity,holm2012collision}.
Human motion prediction (HMP) enables a number of exciting applications such as redirected walking to create the illusion of unlimited virtual interaction spaces~\cite{azmandian2016automated,sun2018towards} or to steer users away from physical boundaries, such as walls, and thus avoid collisions~\cite{gamage2021so,zheng2022gimo}.
Human motion prediction can also provide users with a low-latency experience by preparing VR content in advance based on the predicted future human poses~\cite{hou2019head,9983833} and it has been used to generate human-like motions for virtual agents to enhance the interaction experience~\cite{bhattacharya2021text2gestures,du2023avatars}.

Previous work on HMP has typically generated human motions in a deterministic way, i.e. by producing only a single prediction at a time~\cite{martinez2017human,butepage2017deep,cao2020long,gopalakrishnan2019neural}.
Recently, in light of the fact that human motion is stochastic by nature~\cite{chen2023humanmac, barquero2022belfusion}, researchers have turned to stochastic human motion prediction, i.e. generating a number of reasonable human motions at a time~\cite{chen2023humanmac,yuan2020dlow,barquero2022belfusion,barsoum2018hp}.
Stochastic human motion prediction suits the needs of many VR applications.
For example, to minimise the collision risk in a virtual environment, it is necessary to consider multiple possible future trajectories to warn the users.
To produce realistic virtual agents, it is also beneficial to synthesise multiple reasonable human motions that users can peruse and select from according to their personal preferences.
However, existing stochastic HMP methods typically generate human motions using only past observed motions and neglect other modalities, in particular human eye gaze.
With rapid advances in eye tracking technology, human eye gaze information has become readily available in many VR/AR head mounted displays (HMDs), such as HTC Vive Pro Eye, Varjo VR-3, and Vision Pro, and has demonstrated its potential for gaze-based interaction~\cite{sidenmark2019selection} and gaze-contingent rendering~\cite{hu2019sgaze, hu2020dgaze} in VR/AR.
In addition, a large body of work in the cognitive sciences and human-centred computing has shown that human body movements are closely coordinated with human gaze behaviour~\cite{hu2021ehtask,hu2021fixationnet, sidenmark2019eye, freedman2008coordination}.
Despite this close coordination, information on eye gaze has not been used for stochastic human motion prediction so far.

To address this limitation we propose \textit{GazeMoDiff} -- the first \textbf{Gaze}-guided human \textbf{Mo}tion \textbf{Diff}usion model to generate multiple reasonable human motions.
Our method first uses a 1D convolutional neural network (1D CNN) and a graph attention network (GAT) to extract features from eye gaze and body motion respectively, then employs a spatio-temporal graph attention network to fuse these features, and finally injects the gaze-motion features into a noise prediction network via a cross-attention mechanism to generate multiple reasonable human future motions through a progressive denoising process.
We extensively evaluate our method on the MoGaze dataset~\cite{kratzer2020mogaze} for real-world setting as well as on the GIMO dataset~\cite{zheng2022gimo} for AR setting.
Experimental results demonstrate that our method significantly outperforms the state-of-the-art methods that only use past body poses, achieving an improvement of %12.8\% on MoGaze and 10.6\% on GIMO in terms of average displacement error, 
16.7\% on MoGaze and 10.8\% on GIMO in multi-modal average displacement error and 17.3\% on MoGaze and 13.3\% on GIMO in multi-modal final displacement error.%\zhiming{Give the results on MMADE and MMFDE, also change the results in the abstract}
%Using only historical body poses as input, our method still outperforms prior methods by 9.3\%, 
%in ADE by 9.3\% on MoGaze and 0.4\% on GIMO, 
%demonstrating the effectiveness of our model architecture.
To qualitatively evaluate our method, we further conduct a user study and the responses from $23$ users validate that the motions generated by our method are perceived as both more precise and more realistic than predictions of prior methods.
The full source code and trained models are available at zhiminghu.net/yan24\_gazemodiff.
%~\footnote{Code and pretrained models will be released upon acceptance.}

The main contributions of our work are three-fold:
\begin{itemize}
    \item We propose a novel gaze-guided diffusion model for stochastic human motion prediction that uses a spatio-temporal graph attention network to fuse the gaze and motion features and then injects these features into a noise prediction network via a cross-attention mechanism to generate multiple reasonable human motions in the future.
    
    \item We conduct extensive experiments on two public datasets for both real-world and AR settings and demonstrate significant performance improvements over state of the art.% in terms of both precision and realism.
    
    \item We report a user study that shows the motions generated by our method are perceived as more precise and more realistic than that from prior methods.
\end{itemize}

==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/method.tex <==
\section{GazeMoDiff Model}

Our diffusion model for gaze-guided stochastic human motion prediction takes past body poses and eye gaze information as input.
We represent human pose $p \in \mathbb{R}^{j \times 3} $ using the 3D positions of all human joints, where $j$ denotes the number of human joints.
Eye gaze $g \in \mathbb{R}^{1 \times 3}$ is defined as a unit direction vector. 
Given $H$ frames of observed sequence $\mathbf{x} = [ (g_1, p_1 ), (g_2, p_2),...,(g_H, p_H) ]$, our goal is to predict human motions in the future $F$ frames.
Considering the stochastic nature of human motion, we generate $k$ different future motion trajectories to provide multiple reasonable predictions $\mathbf{P} = \{ \mathbf{p}_{0}, \mathbf{p}_{1},..., \mathbf{p}_{k} \}$, where $\mathbf{p}_{i} = [p_{H+1}, p_{H+2}, ..., p_{H+F}]$. 
%to train a model that can predict $k$ different following $F$-frame future human motions. 
%It can be formulated as $\mathbf{P} = f_p(\mathbf{x},k)$, where $\mathbf{p} = \{ \mathbf{p}_{0}, \mathbf{p}_{1},..., \mathbf{p}_{k} \}$ and $\mathbf{p}_{i} = [p_{H+1}, p_{H+2}, ..., p_{H+F}]$.
An overview of our model is shown in \autoref{fig:pipeline}.
%\andreas{this shouldn't be a table of contents -- directly explain the model/approach high-level (its main components). The following subsecions then go into detail. Here you can also refer to the method figure.}
Our model consists of three modules: a gaze-motion feature extraction module that uses a gaze encoder and a motion encoder to extract gaze and motion features respectively, a gaze-motion feature fusion module that fuses the gaze-motion features using a spatio-temporal graph attention network, as well as a diffusion-based motion generation module that employs a cross-attention mechanism to inject the gaze-motion features into a noise prediction network to generate multiple reasonable human future motions through progressive denoising.
%At a high level, our model consists of a gaze encoder and a pose encoder to extract features within the same modality, a cross-modal fusion module to fuse human gaze and motion features as well as a motion generation module.
%\zhiming{better to explain right after you use it.}
%, $H$ and $F$ denote the number of human joints, the time window of historical observation, and the time window of future prediction, respectively. Our model is stochastic and can generate $K$ different predictions $\mathbf{p}_0, \mathbf{p}_1, ..., \mathbf{p}_K$ %\zhiming{You need to emphasise that is generate multiple predictions for one time point. Here it is not so clear.}.
%In this section, we first detailed and clearly articulated the problem definition. Then we introduced 
%\zhiming{past sense}
%the \hl{ST-GAT} for capturing correlations and fusing features
%\zhiming{Throughout the paper (abstract, into, conclusion), you can simply say ``gat for fusing motion and gaze features'' for simplicity.}
%and our denoising network for predicting noise. Finally, we show our training and inference pipeline.
%\zhiming{followed by $->$ following. No need to mention this here.}. 


\begin{figure*}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=2\columnwidth]{figs/Visio-pipeline_new_new.pdf}
 \caption{Overview of the proposed method \textit{GazeMoDiff}.
 \textit{GazeMoDiff} first uses a gaze encoder and a motion encoder to extract the gaze and motion features respectively, then employs a spatio-temporal graph attention network to fuse these features, and finally injects the gaze-motion features into a noise prediction network via a cross-attention mechanism to generate multiple reasonable human future motions through a progressive denoising process.
 %\textit{GazeMoDiff} first uses a gaze encoder and a motion encoder to extract features from eye gaze and human motions. A spatio-temporal graph attention network then integrates them into cross-modal features, then injects these features into a noise prediction module via a cross-attention mechanism, and finally generates multiple reasonable human motions through progressive denoising.
 %extracts and fuses features from gaze and motion data 
 %A Gaze-motion Fusion module extracts the features from gaze and motion input. The gaze-motion features are injected into a noise prediction module via a cross-attention mechanism to generate realistic motions by progressive denoising. %\hl{LN, SA and CA denote layer normalisation, self-attention block and cross-attention block.}%\zhiming{Here, it seems like the noise prediction and completion denoising mechanism are two distinct parts. However, in the figure, these two parts are coupled in the Noise Prediction Network. Also, the input and output take too much space in the figure. You can make them much smaller because they don't convey any important information. You can use the space for the details of your main novelty, especially the structure of the GAT. Actually, the Noise Prediction Network should be Noise Prediction and Denoising Network, right?}
 %\zhiming{This figure is too small, better to use double column. Use pdf format (bit map) is better than png (pixel map). You need to explain the pipeline of the method in the caption.}
 }
 \label{fig:pipeline}
\end{figure*}




%\subsection{Problem Definition}
\subsection{Gaze-motion Feature Extraction}

\subsubsection{Gaze Encoder}
%\zhiming{first pad H->H+F, following prior works[x]}
We first pad raw observed gaze data $G_{raw} \in\mathbb{R}^{{3}\times{1} \times {H}}$ to full-length gaze data $G \in\mathbb{R}^{{3}\times{1} \times {(H+F)}}$ following prior work ~\cite{chen2023humanmac}.
We then employed an approximate discrete cosine transform (DCT)~\cite{mao2021generating} that selected the first $L$ components to process the full-length gaze data $G \in\mathbb{R}^{{3}\times{1} \times {(H+F)}}$.
By leveraging this transformation, the time dimension of eye gaze signals was reduced from $H+F$ to $L$, which both improved the smoothness of generation and reduced computational complexity~\cite{mao2019learning}. 
We further employed a 1D convolutional neural network as an encoder to extract features from the transformed eye gaze sequence $G_{dct} \in\mathbb{R}^{{3}\times{1} \times {L}}$.
%of the DCT gaze sequence. % , which has shown promise for processing sequence direction vectors, e.g, gaze \cite{hu2020dgaze} and head orientation \cite{hu2021fixationnet,hu2021ehtask}.
Specifically, we used four CNN layers with the kernel size of three.
The channel size of the first three layers is $32$ and each layer is followed by a layer normalisation (LN) and a Tanh activation function.
After the three CNN layers, we employed an extra CNN layer with three channels and a Tanh activation function to obtain the final eye gaze feature $f_{gaze}\in\mathbb{R}^{{3}\times{1} \times {L}}$.

\subsubsection{Motion Encoder}
%\zhiming{The data follow in this encoder is not clear.}
Recent works have demonstrated that a graph structure is particularly effective for learning 
%a natural representation of the human pose, is particularly effective for learning
inherent correlations between human body joints~\cite{li2021directed,li2021multiscale,ma2022progressively}.
%Previous work on graph attention networks (GATs) has shown good results for human pose aggregation \cite{velivckovic2017graph}. 
Inspired by these works, %\zhiming{first pad H->H+F, following prior works[x]} 
we treated human motions as a fully-connected spatio-temporal graph $P \in \mathbb{R}^{3 \times j \times (H+F)}$, where later $F$ frames of poses were padded with the last observed frame. 
Similarly, we employed DCT to obtain the transformed spatio-temporal graph $P_{dct} \in\mathbb{R}^{3 \times j \times L}$ for smoother generation and lower computational complexity. 
We designed a GAT-based motion encoder to model the spatio-temporal correlations in the motion sequence for extracting motion features $f_{motion}\in\mathbb{R}^{{3} \times j \times {L}}$.
The motion encoder consisted of three GAT blocks i.e. a
start GAT block, a middle GAT block, and an end GAT block. %The attention head of each spatial GAT layer and temporal GAT layer was set to eight
%Each GAT block contained a temporal GAT layer, a spatial GAT layer, a linear layer, a layer normalisation, a Tanh activation function as well as a dropout layer with a 0.3 dropout rate.
%The attention head of each spatial GAT layer and temporal GAT layer was set to eight.
%The output feature dimensions of the start, middle, and end 
%\zhiming{here, it is difficult to understand start, middle, and end (they are not explained before) without a figure}
%layers were 16, 16, and 3, respectively.

\textbf{Start GAT Block}. 
Given the transformed spatio-temporal graph $P_{dct}\in\mathbb{R}^{3 \times j \times L}$,  
%\zhiming{H is not explained before. The data flow is not clear. We have X, Y, but what's H} of each block\zhiming{'block' is not explained},
%where $f$ is the feature dimension of input, 
we first enhance the features using a multi-head self-attention mechanism via the temporal GAT layer%\zhiming{aggregated features along a dimension usually means reducing that dimension} 
and obtained $H^{\prime} =[{h}_1^{\prime},{h}_2^{\prime},...,{h}_L^{\prime}] \in\mathbb{R}^{3 \times j \times L}$ in the following way:

\begin{equation}
    {h}_i^{\prime}=\operatorname{LeakyReLU}\left(\frac{1}{N_{head}} \sum_{n=1}^{N_{head}} \sum_{k =1}^{L} \alpha_{i k}^n  {h}_k\right),
\end{equation}
where $ {h}_i^{\prime} \in\mathbb{R}^{3 \times j} $ is the output feature of node $i$, ${h}_k$ is the input feature of node $k$, and $N_{head}=8$ denotes the number of heads for attention.
We fused different output features from each head by averaging them.
For each head, the attention matrix $\alpha_{i k}^n$ represents interactions between each timestamp, calculated as follows: 
\begin{equation}
    \alpha_{i k}^n =\frac{\exp \left(\operatorname{LeakyReLU}\left({\mathbf{a}^n}\left[ {h}_i \oplus  {h}_k\right]\right)\right)}{\sum_{l=1}^{T} \exp \left(\operatorname{LeakyReLU}\left({\mathbf{a}^n}\left[ {h}_i \oplus  {h}_l\right]\right)\right)},
\end{equation}
where ${\mathbf{a}^n}$ is a parameter vector $\in \mathbb{R}^{6 \cdot j \times 1}$ and $\oplus$ denotes concatenation operation. 

A linear layer was then used to transfer feature dimension from $H^{\prime} \in\mathbb{R}^{3 \times j \times L}$ to $\Bar{H}^{\prime} \in\mathbb{R}^{16 \times j \times L}$.%\zhiming{what's $f^{\prime}$?}
%.
We further proposed a spatial graph attention network layer to extract features between different joints and obtain the output of the start GAT block $H_{sta} \in\mathbb{R}^{16 \times j \times L}$. Specifically, the spatial GAT layer was similar to the temporal GAT layer
%\zhiming{'temporal GAT layer' is not mentioned before}
, differing primarily in how attention coefficients were computed. Rather than extracting features in the temporal dimension as in the temporal GAT, the spatial GAT extracts features across the spatial dimension. 

\textbf{Middle GAT Block}.
We designed a middle GAT block to further extract the body pose features. Taking the output of the Start GAT block $H_{sta} \in\mathbb{R}^{16 \times j \times L}$ as input, we first duplicated the temporal features for enhancement~\cite{ma2022progressively} $\left(\mathbb{R}^{16 \times j \times L}\rightarrow \mathbb{R}^{16 \times j \times 2L} \right)$. Then we used a temporal GAT layer, a linear layer, and a spatial GAT layer to further learn correlations between joints and extract features. Note that the input and output dimensions of the linear layer in the middle GAT block are both 16. Then a layer normalisation, a Tanh
activation function, and a dropout layer with 0.3 dropout rate was used after the spatial GAT layer to avoid overfitting. A skip connection was added to improve the network flow.
%between of the input of temporal GAT layer and the output of the spatial GAT layer for easier optimisation.
To keep the temporal dimension of the original input to this block the same, the middle GAT block's output $f_{mid}$ was divided in half in the temporal dimension $\left(\mathbb{R}^{16 \times j \times 2L}\rightarrow \mathbb{R}^{16 \times j \times L} \right)$.

\textbf{End GAT Block}. The end GAT block was used to obtain the final motion features with the same feature dimension in gaze features $f_{gaze}$ for further fusion. This block consists of a temporal GAT, a linear layer (reducing feature dimension from 16 to 3), a spatial GAT, a layer normalisation (LN), a Tanh
activation function, and a dropout layer with 0.3 dropout rate.
Given $f_{mid} \in \mathbb{R}^{16 \times j \times L}$, the end GAT block outputs $f_{motion}\in \mathbb{R}^{3 \times j \times L}$.

\subsection{Gaze-motion Feature Fusion}
%The human pose is represented as a series of coordinate values\zhiming{a series of coordinate values? 3D positions} of the human joints. 

%Different from prior works, 

To fuse gaze and motion features, we treated gaze and motion features as ``virtual joints'' and combined gaze and poses together as a fully connected graph $f_{in} \in \mathbb{R}^{3 \times (j+1) \times L}$. Then a similar spatio-temporal GAT was employed to fuse gaze and motion features.

The gaze-motion fusion module was composed of a start GAT block, four middle GAT blocks, and an end GAT block. The structures of those blocks are the same as the blocks in the motion encoder.
The gaze-motion features $f_{fus} \in \mathbb{R}^{3 \times (j+1) \times L}$ were calculated as:
\begin{equation}
    \label{gazemotionfuse}
    f_{fus} = GazePoseFuse \left(f_{in}\right).
\end{equation}

%\andreas{explain things in the correct order, step by step. "before" should never occur/be required}
%Before constructing this graph structure, 

%\zhiming{Any references?}. 
%Given the original spatio-temporal graph $X \in \mathbb{R}^{3 \times (j+1) \times (H+F)}$, the DCT spatio-temporal graph $Y \in\mathbb{R}^{3 \times (j+1) \times L}$ was obtained by DCT.
%\zhiming{the spatio-temporal graph $Y \in\mathbb{R}^{3 \times (j+1) \times L}$ can be concatenated along the spatial dimension? What does this mean?}.\reply{I've changed the expression to make it easy to get.} 
%From a temporal perspective, the graph contains $T$ nodes $X_1, X_2, ..., X_L \in\mathbb{R}^{3 \times (j+1) }$ and the edges between them indicate correlations between each timestamp. From another spatial perspective, the graph contains $j+1$ nodes $X^1, X^2, ..., X^{j+1}$, and the edges between them represent correlations between each joint (gaze also can be regarded as a joint).


%We designed the Gaze-motion Fusion module ${GazePoseFuse}\left(\cdot\right)$, illustrated in \autoref{fig:pipeline}, to model the spatio-temporal correlations in the defined graph and fuse the gaze-motion features.
%The Gaze-motion Fusion module was composed of a stack of temporal GAT layers and spatial attention GAT layers with skip connections.
%In this module, the number of middle blocks $m$ is 4 and there is a layer normalisation, tanh activation function and a dropout layer after each middle block. The attention head of each spatial GAT layer and temporal GAT layer is 8. The output feature dimension of the start, middle, and end block is 16, 16, and 3, respectively. The gaze-motion feature is calculated as:
%\begin{equation}
%    \label{gazemotionfuse}
%    H^{\prime\prime} = GazePoseFuse \left(Y\right)
%\end{equation}

%We only introduce the temporal GAT layer and spatial GAT layer here for brevity.
%$\andreas{not sure what the last sentence tries to say. Explain what needs to be explained, at the required level of detail. if something is not required then move to appendix or leave out completely.} 
%Given the input $H \in\mathbb{R}^{f \times (j+1) \times L}$ of each block, where $f$ is the feature dimension of input, we first aggregated features along the temporal dimension and obtain $H^{\prime} =[{h}_1^{\prime},{h}_2^{\prime},...,{h}_L^{\prime}] \in\mathbb{R}^{f \times (j+1) \times L}$ in the following way:

%\begin{equation}
%    {h}_i^{\prime}=\operatorname{LeakyReLU}\left(\frac{1}{N_{head}} \sum_{n=1}^{N_{head}} \sum_{k =1}^{L} \alpha_{i k}^n  {h}_k\right)
%\end{equation}
%where $ {h}_i^{\prime} \in\mathbb{R}^{f \times (j+1)} $ is the output feature of node $i$, ${h}_k$ is the input feature of node $k$, and $N_{head}$ denotes the number of heads for attention.
%We fused different output features from each head by averaging them.
%For each head, the attention matrix $\alpha_{i k}^n$ represents interactions between each timestamp, calculated as follows: 
%\begin{equation}
%    \alpha_{i k}^n =\frac{\exp \left(\operatorname{LeakyReLU}\left({\mathbf{a}^n}\left[ {h}_i \oplus  {h}_k\right]\right)\right)}{\sum_{l=1}^{T} \exp \left(\operatorname{LeakyReLU}\left({\mathbf{a}^n}\left[ {h}_i \oplus  {h}_l\right]\right)\right)}
%\end{equation}
%where ${\mathbf{a}^n}$ is a parameter vector $\in \mathbb{R}^{2f(j+1) \times 1}$ 

%A weigh matrix $\mathbf{W} \in \mathbb{R}^{f \times f^{\prime}}$ was then used to transfer feature dimension from $H^{\prime} \in\mathbb{R}^{f \times (j+1) \times L}$ to $\Bar{H}^{\prime} \in\mathbb{R}^{f^{\prime} \times (j+1) \times L}$.

%To further capture correlations between joints and the gaze feature, we proposed a spatial graph attention network layer. Specifically, the spatial GAT layer was in a similar manner to the temporal GAT layer, differing primarily in how attention coefficients were computed. Rather than aggregating along the temporal axis as in the temporal GAT, the spatial GAT aggregated features across spatial dimensions as follows: 

%\begin{equation}
%{h}_i^{\prime\prime}=\operatorname{LeakyReLU}\left(\frac{1}{ \Bar{N}_{head}} \sum_{n=1}^{ \Bar{N}_{head}} \sum_{k =1}^{j+1} \Bar{\alpha}_{i k}^n   \Bar{h}_k^{\prime}\right)
%\end{equation}
%where $ {h}_i^{\prime\prime} \in\mathbb{R}^{f^{\prime} \times L } $ is the output feature of node $i$ and $\Bar{N}_{head}$ denotes the number of heads for attention. We also applied an average function to fuse different output features from each head in spatial GAT. For each head, the attention matrix $\Bar{\alpha}_{i k}^n$ represents interactions between each timestamp, calculated as follows: 
%\begin{equation}
%    \Bar{\alpha}_{i k}^n =\frac{\exp \left(\operatorname{LeakyReLU}\left({\Bar{\mathbf{a}}^n}\left[ \Bar{h}_i^{\prime} \oplus  \Bar{h}_k^{\prime}\right]\right)\right)}{\sum_{l=1}^{j+1} \exp \left(\operatorname{LeakyReLU}\left({\Bar{\mathbf{a}}^n}\left[ \Bar{h}_i^{\prime} \oplus  \Bar{h}_l^{\prime} \right]\right)\right)}
%\end{equation}
%where $\Bar{\mathbf{a}}^n$ is a parameter vector $\in %\mathbb{R}^{2f^{\prime} L \times 1}$ 

%The spatio-temporal graph attention module is detailed above. The final gaze-motion fusion network\zhiming{final? gaze-motion fusion network is one network/module from your figure.}, ${GazePoseFuse}\left(\cdot\right)$, is a stack of such modules with the residual connection\zhiming{It is necessary to visualise this structure briefly in the figure. Otherwise it is difficult for people to image. Also because this is your main novelty. Also you have the space for this. Make the box for gaze-pose graph and gaze-motion features one column to save more space.}. The gaze-motion feature is calculated as:

\subsection{Diffusion-based Motion Generation}
%\zhiming{Noise Prediction Network, be consistent with the use of upper/smaller case.}
%Prior work \cite{chen2023humanmac} introduced observation via simple addition\zhiming{observation via simple addition?}, which does not fully leverage dependencies between observation\zhiming{make it clear observation means the input.} and noisy predictions.
%\zhiming{Just say prior work, no need to mention the name. Otherwise, it raises the question why not compare with this method?}
%\hl{Given the gaze-motion features $H^{\prime\prime}$ derived by the Gaze-motion Fusion module, we apply a noise prediction module for }
We formulated the motion generation task as an inverse diffusion process, which contains iterative noise prediction and denoising steps.

\textbf{Noise prediction.} Inspired by text-driven noise prediction network~\cite{zhang2022motiondiffuse}, we designed a noise prediction network
%\zhiming{in which aspect your network is inspired by that work? it seems noise prediction network is a general term in diffusion model and the characteristic of your noise prediction network is not clear} 
${\boldsymbol{\epsilon}_\theta}$ that employed the cross attention mechanism to guide the denoising process using the gaze-motion features. This network is developed to predict the noise at the current time step given the gaze-motion features $f_{fus}$ and noisy motion sequence $Y^t\in\mathbb{R}^{3 \times (j+1) \times L}$ from the previous time step. As illustrated in~\autoref{fig:pipeline}, ${\boldsymbol{\epsilon}_\theta}$ consists of $n$ stacked self-attention block, cross-attention block and multi-layer perception (MLP) block with skip connections.%\zhiming{skip connections are not shown in the figure}. 
 Additionally, to trade off diversity and realism of predictions, we train our model using classifier-free guidance~\cite{ho2022classifier}. 
Specifically, the model predicted noises from both conditional and unconditional prior by randomly setting $c = None$ for 10\% possibility and $c = f_{fus}$ for 90\% possibility. 
The predicted noise at time step $t$ is formulated as follows:
\begin{equation}
   \label{nosieprediciton}
   \Bar{\boldsymbol{\epsilon}} =  \boldsymbol{\epsilon}_{\boldsymbol{\theta}}\left( Y^t, c, t\right).
\end{equation}
%\zhiming{there is a gap between last paragraph and this one. Since you use a separate paragraph to introduce this, you can emphasise this in your method figure.} 

To better model the temporal correlations within the noisy gaze-motion sequence $Y^t \in \mathbb{R}^{3 \times (j+1) \times L}$, we first employed a linear transformation to project the sequence into a higher-dimension latent space $Y^{\prime t} \in \mathbb{R}^{3 \times (j+1) \times L^{\prime}}$. We then applied an efficient self-attention block\cite{zhang2022motiondiffuse} to further model temporal correlations between each frame, $\mathbf{Y} = \operatorname{self-att}\left( Y^{\prime t} \right) +  Y^{\prime t}$

%\begin{equation}
%    \mathbf{Y} = \operatorname{Dropout}\left(\operatorname{softmax}\left( \mathbf{Q} \right) \operatorname{softmax}\left( \mathbf{K}^\top \right)\right)\operatorname{LN}\left(\mathbf{V}\right) +  Y^{\prime t},
%\end{equation}
%where $\operatorname{LN}$ is layer normalisation,  $\mathbf{Q}\in\mathbb{R}^{L\times d}$, $\mathbf{K}\in\mathbb{R}^{L\times d}$, and $\mathbf{V}\in\mathbb{R}^{L\times d}$ are calculated using the original self-attention mechanism\cite{vaswani2017attention}:
%\begin{equation}
%    \mathbf{Q} = \mathbf{W}_q  Y^{\prime t}, \mathbf{K} = \mathbf{W}_k  Y^{\prime t},\mathbf{V}  \mathbf{W}_v Y^{\prime t},
%\end{equation}
%where  $\mathbf{W}_q$, $\mathbf{W}_k$ and $\mathbf{W}_v$ are learnable parameter matrices. 
%Then instead of computing element-wise attention (
%$\mathcal{O}\left(L^2d \right)$), linear attention \cite{shen2021efficient} ($\mathcal{O}\left(d_kdL \right)$ where ${d_k}$ denotes feature dimension spilt by the number of multi-head) is calculated as:
%It %\zhiming{This modelling?} 
%enables a global perceptual vision of the whole sequence temporally and thus is beneficial for following modality fusion and noise prediction \cite{zhang2022motiondiffuse}. Besides, to overcome the high computational complexity of the attention mechanism, we adopt an efficient version
%\zhiming{How is it efficient? in which way? A paper should contain everything in itself.}\reply{I compared the time complexity of this version and you can see the equation of computing attention is different from the original self-attention in the transformer}
%\cite{shen2021efficient}. 



We then applied a step hint module to inform about how many steps of noise have been added thus far. We first obtained the timestep embedding $\mathbf{e}_t$ using position embedding\cite{vaswani2017attention}. The gaze-motion historical features $c$ were also fused with a learned linear projection of the timestep embedding, $\mathbf{e} = \mathbf{e}_t + \mathbf{W}^\prime c$. This fused embedding $\mathbf{e}$ was then injected into the output of the self-attention block, $\mathbf{Y}^{\prime} = \operatorname{step-hint}\left(\mathbf{Y},\mathbf{e}\right)$.% using a feature-wise linear modulation:

%\begin{equation}
%   w = \phi_w\left(\psi\left( \mathbf{e}_t \right)\right), \ b = \phi_b\left(\psi\left( \mathbf{e}_t \right)\right), \ \mathbf{Y}^{\prime} = \operatorname{SiLU}\left(w\cdot\mathbf{Y} + b\right),
%\end{equation}
%where $\left(\cdot\right)$ denotes element-wise multiplication, $\phi_w$ and $\phi_b$ are linear projections, and $\psi$ is a single layer MLP with SiLU activation function. This modulation allowed the step hint embedding to influence the self-attention features. We also applied this block after each cross-attention and MLP block, enabling the timestep embedding to provide hints throughout the network.
%To bring these hints into the noise prediction network, we applied step hint blocks after every self-attention, cross-attention and FFN block. We first obtain the timestep embedding $\mathbf{e}_t$ by position embedding\cite{vaswani2017attention} and the gaze-motion historical features $H^{\prime\prime}$ is also summed with fused embedding $\mathbf{e} = \mathbf{e}_t + \operatorname{Linear}\left(H^{\prime\prime}\right)$. This fused embedding $\mathbf{e}$ then is injected into the output of each block:


%\zhiming{Again, there is a gap here. You should make the data flow more clear and explain which blocks are used for which data.} 
To incorporate the historical gaze-motion features
$f_{fus}$
%$H^{\prime\prime}$
%\zhiming{$H^{\prime\prime}$ does not correspond with 3.2} 
and leverage their impact on noise prediction, we utilised cross-attention blocks. These blocks enable a deeper exploration of how the historical features influence the noise predictions at different denoising steps. In addition, computing the contributions of different attention heads in parallel better integrates information from both modalities (gaze and motion). % from multiple perspectives\zhiming{from both modalities (gaze and motion) from multiple perspectives?}.
Potentially, the noisy motions can also provide feedback to update $c$, leading to a collaborative learning process. In the cross-attention block, $\mathbf{Q}_c$  and $\mathbf{V}_c$ were calculated by gaze-motion historical features $c$ while $\mathbf{K}_c$ was calculated using the output of self-attention blocks $\mathbf{Y}^\prime$. The output of the cross-attention block was calculated as follows:
\begin{equation}
  \mathbf{Y}_c = \operatorname{Dropout}\left(\operatorname{softmax}\left( \mathbf{Q}_c \right) \operatorname{softmax}\left( \mathbf{K}_c^\top \right)\right)\operatorname{LN}\left(\mathbf{V}_c\right)+ \mathbf{Y}^\prime.
\end{equation}
\begin{equation}
     \mathbf{Q}_c = \mathbf{W}^\prime_q  c, \mathbf{K}_c = \mathbf{W}^\prime_k  \mathbf{Y}^\prime,\mathbf{V}_c = \mathbf{W}^\prime_v  c.
\end{equation}

Finally, we employed a two-layer MLP with GELU activation function and a dropout layer with 0.2 dropout rate 
%\zhiming{what's the dropout rate} 
to further extract features. A linear layer  %\zhiming{projection layer? linear layer?} 
was added at the end to align with the noise dimension.

 %\zhiming{Is this the completion denoising? If not, you don't have a specefic paragraph for completion denoising. Make the block name match the name in the method figure.} 

In our implementation, the noise prediction network contained four self-attention blocks, four cross-attention blocks, and four MLP blocks. Each attention operation used eight attention heads. The timestep embedding dimension and the latent space dimension were both set to 512.

\textbf{Denoising.} %In the inference stage
%\zhiming{Somewhere earlier (beginning of the method section), you should emphasise that you have two stages. Otherwise people don't know what is the inference stage.}
%, the full gaze-motion sequence $X$ is unavailable while only the observed gaze-motion sequence $X_{obs}$ is given. 
In a vanilla approach, the denoised sequence was generated directly from the Gaussian noise input. 
However, due to the accumulation of prediction noise errors, the observation information in the padded sequence is far from the truth in the latter steps. 
In each denoising step, the observed sequence was also available to guide the generation in the original space. Thus, we employed an ingenious prediction mask mechanism~\cite{chen2023humanmac} to obtain denoised motions $\mathbf{\Bar{p}} \in \mathbb{R}^{3 \times j \times F}$ progressively. The detailed denoising process is illustrated in the supplementary material. 
%\zhiming{no need to give so many details of the mask mechanism since it is not your contribution}:

%Following
%\zhiming{Following by?} 
%\cite{chen2023humanmac}, the trained model can generate diverse predictions in a completion denoising mechanism. 

%\textbf{Adding noises into the padded sequence.}
%First, the padded gaze-motion sequence in DCT domain $\Bar{Y}$ is obtained in \autoref{Ypred}. Then, the noisy input at timestep $t$ can be calculated by:

%\begin{equation}
%    \Bar{Y}^t = \sqrt{\bar{\beta}_t}\Bar{Y} +\sqrt{1-\bar{\beta}_t} \boldsymbol{\epsilon}
%\end{equation}

%The detailed training and inference procedure is illustrated in the supplementary material.
%\zhiming{details of what?}



\subsection{Training}
%\zhiming{These small subsubsections can be used as paragraphs.}
%Current diffusion-based HMP methods could be divided into two fashions: 1) Trained to generate the prediction motion sequence, it can be used to generate prediction motion sequences directly in the inference stage. \cite{barquero2022belfusion,saadatnejad2023generic} 2) Trained to generate the whole motion sequence (observation and prediction), the prediction sequence can be obtained by completion denoising, \cite{chen2023humanmac}, which has demonstrated better motion consistency, prediction accuracy, and a more straightforward end-to-end training pipeline without a painstakingly designed loss function is proposed. Thus, we followed the latter approach. 
%We followed the training and inference pipeline of \cite{chen2023humanmac} as it has demonstrated better motion consistency, prediction accuracy, and a more straightforward end-to-end training pipeline without a painstakingly designed loss function. Trained to generate the whole motion sequence (observation and prediction), the prediction sequence can be obtained by the completion denoising mechanism.
%\zhiming{The following three paragraphs are completion denoising mechanism, right? Then you should bold completion denoising mechanism rather than the three steps so that people can easily find it.} \reply{No. Completion denoising only used in inference stage.}

In the training stage, the observation and prediction sequences are both available. Thus, we trained the model on the full-motion sequence $X_{full} \in \mathbb{R}^{3 \times (j+1) \times (H+F)}$ . First, we also transferred $X_{full}$ into the DCT space $Y_{full} \in \mathbb{R}^{3 \times (j+1) \times L}$. We then added noise to $Y_{full}$ to generate a noisy sequence $Y_{full}^{t}$. Then we predicted the noise through \autoref{nosieprediciton}.

We then optimised all parameters in our pipeline by minimising the $l_2$ %\zhiming{be consistent with $l_2$ or L2 throughout the paper} 
loss between the predicted noise $\boldsymbol{\epsilon}_{\boldsymbol{\theta}}\left( Y^t, c, t\right)$ and the true noise $\epsilon$:
\begin{equation}
    \mathcal{L}=\mathbb{E}_{\boldsymbol{\epsilon}, t}\left[\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_{\boldsymbol{\theta}}\left( Y_{full}^t, c, t\right)\right\|^2\right].
\end{equation}

The detailed training and inference procedure is illustrated in the supplementary material.

%The detailed training procedure is shown in the supplementary material.


%\textbf{Adding noises to the transformed sequence.} The diffusion model is trained by predicting noises in noisy input step by step. The noisy gaze-pose graph $Y^t\in\mathbb{R}^{3 \times (j+1) \times L}$ is calculated by:

%\begin{equation}
%    Y^t=\sqrt{\bar{\beta}_t}Y^0 +\sqrt{1-\bar{\beta}_t} \boldsymbol{\epsilon}
%\end{equation}

%\begin{equation}
%    \bar{\beta}_t=\prod_{i=1}^t \beta_i, \beta_i \in[0,1]
%\end{equation}

%\textbf{Obtaining gaze-motion conditional feature.} Then we employ the aforementioned noise prediction network outputs the predicted noise ${\boldsymbol{\epsilon}_\theta (Y^t, H^{\prime\prime}, t)}$ given original observation sequence (including gaze) at timestep $t$, where $H^{\prime\prime}$ is the output of ${GazePoseFuse}$:

%\begin{equation}
%    H^{\prime\prime} = {GazePoseFuse}\left(Y_{obs}\right)
%\end{equation}
%\begin{equation}
%    Y_{obs} = \operatorname{DCT}\left(\operatorname{Pad}\left(X_{obs}\right)\right)
%\end{equation}
%where $X_{obs} \in\mathbb{R}^{3 \times (j+1) \times H}$ denotes the original gaze-motion sequence and  $\operatorname{Pad}\left(\cdot\right)$ pads the $F$-frame poses with the last frame's pose ($\mathbb{R}^{3 \times (j+1) \times H} \rightarrow \mathbb{R}^{3 \times (j+1) \times (H+F)}$ ). 

%\textbf{Predicting the noise.} 





==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/related_work.tex <==
\section{Related Work}

\subsection{Human Motion Prediction}
Human motion prediction is a fundamental research topic in virtual and augmented reality.
Early studies commonly considered HMP as a deterministic sequence prediction task, tackling it with recurrent neural network (RNN)~\cite{martinez2017human,ghosh2017learning,li2017auto,fragkiadaki2015recurrent},
%.  However, due to the structure of RNN, it is prone to error accumulation and gradient vanishing, which can yield inaccurate and discontinuous results. Then, there are some approaches with \hl{elaborate loss function} based on adversarial networks\cite{kundu2019bihmp,barsoum2018hp}, 
graph neural network (GNN)~\cite{li2021directed,li2021multiscale, hu24hoimotion} and Transformers~\cite{aksan2021spatio,martinez2021pose}. 
%emerging and achieving \hl{better results}. 
%In parallel to trying out ingenious frameworks, other works \cite{corona2020context,zheng2022gimo} have attempted to improve the performance by incorporating multimodal information (
%$e.g.$ gaze \cite{zheng2022gimo} 
%and context objects \cite{corona2020context}) beyond the historical human pose sequence. This fits more naturally with the logic of human prediction, which is determined by a synergy of his past motions, surroundings, intentions, and action semantics. 
Noticing that human body motions are inherently stochastic, recent works began to predict human motions in a stochastic way using generative models such as variational autoencoder (VAE)~\cite{aliakbarian2021contextually,mao2021generating}, generative adversarial network (GAN)~\cite{kundu2019bihmp,barsoum2018hp,jain2020gan}, and Flow networks~\cite{yuan2020dlow}.
These methods can generate diverse human motions through a diversity-aware loss or sampling strategy~\cite{mao2021generating,yuan2020dlow}, but their predictions are not physically plausible.
%It meets the demands of many VR applications such as collision warning during human-human interaction and human-environment interaction.
%However, human motions are naturally spontaneous and unpredictable, and a deterministic prediction could be not suitable for a situation where all possible motions are crucial. Different from the above approaches, stochastic HMP methods try to predict diverse possible and reasonable motions. 
%These methods often design a diversity-aware loss or sampling strategy to enforce diversity~\cite{mao2021generating,yuan2020dlow}. 
%However, their predicted sequences were not physically plausible.
Inspired by the recent success of denoising diffusion models in the field of image generation~\cite{ho2020denoising,ramesh2022hierarchical,nichol2021glide,zhang2023adding}, researchers have adopted diffusion models to the task of stochastic human motion prediction and have achieved more realistic predictions than traditional generative approaches~\cite{barquero2022belfusion,chen2023humanmac}.
However, existing methods only generate future motion predictions based on observed past motion, neglecting the fact that human eye gaze is known to correlate strongly with body movements and is readily available in recent VR/AR headsets.
To fill this gap, in this work we propose the first gaze-guided diffusion model for stochastic human motion prediction.
%our work introduces a naturally available modal, gaze, into a diffusion-based model for the first time.


\subsection{Correlations between Eye Gaze and Body Motion}

Intuitively, a period of human eye gaze information seems related to human intention~\cite{koochaki2018predicting}, which can drive future motion trends. Extensive works in cognitive science and human-centred computing have also demonstrated this strong correlation between human eye gaze and subsequent body motion. %\cite{kothari2020gaze,hu2019sgaze,sidenmark2019eye,emery2021openneeds} have revealed how and to what extent gaze can influence the future movements of different parts (e.g., head, hand, torso) of the body. 
%\zhiming{Use ``A et al. [1] propose '' rather than ``[1] propose ''. Don't use citations as the beginning of a sentence.}
Some researchers have revealed that in many everyday activities, such as free viewing or object searching, human head movements are closely associated with eye movements~\cite{zangemeister1982gaze,hu2019sgaze,kothari2020gaze, hu24pose2gaze}.
Emery et al. further explored the coordination of human eye, hand, and head movements in virtual environments and leveraged this coordination to improve the performance of gaze estimation~\cite{emery2021openneeds}.
Sidenmark et al. identified the coordinated movements between eye, head, and torso during gaze shifts in virtual reality~\cite{sidenmark2020bimodalgaze,sidenmark2019eye}.
%\textcolor{red}{Zheng et al. \cite{zheng2022gimo} used eye gaze to filter information from the full 3D scene environment and then employed the scene features for deterministic human motion prediction.}
Despite the strong link between human eye gaze and body motion, prior work has only explored to use eye gaze to filter information from the full 3D scene environment and then employed the scene features for deterministic human motion prediction~\cite{zheng2022gimo}.
%the effectiveness of eye gaze information for stochastic human motion prediction has not been explored so far.
We are the first to directly leverage eye gaze information (without requiring information about the full 3D environment) to further boost the performance of stochastic human motion prediction.

%Although the aforementioned works have indicated the strong relationship between eye movements and human motion trends, existing stochastic HMP methods have not considered this correlation yet.
%We are the first to demonstrate this correlation between gaze and motion, which enhances the realism and trustworthiness of stochastic HMP. This correlation ultimately leads to superior quantitative performance. 
%We are the first to leverage the correlation between gaze and motion, which enhances the realism and trustworthiness of stochastic HMP. This gaze-motion correlation ultimately leads to superior quantitative performance, as we show in this work.
%.
%the spatial and temporal interactions between gaze sequence and pose sequence have not been well studied. 
%can enhance the realism and trustworthiness of stochastic HMP and lead to superior quantitative performance.

%\hl{Inspired by the work\cite{zhao2020multivariate,yan2023graph} in multivariate time-series using graph attention network to capture the correlations between different channels at different timestamps,} We proposed a spatial-temporal graph attention network to model the correlations between coordinates of joints and gaze in each timestamp and demonstrated such a full fusion could improve the performance significantly.
%\zhiming{1. Eye-body correlations have been found by many works, give many examples on this 2. eye gaze has not been used for stochastic HMP 3. we are the first to do so. PS: No need to mention GIMO paper because otherwise people would think your idea is not novel. Refer to the GazeMotion paper.}


\subsection{Denoising Diffusion Models}

Denoising diffusion models, or more precisely, denoising diffusion probabilistic models (DDPM)~\cite{ho2020denoising,song2020denoising,dhariwal2021diffusion,rombach2022high} are a group of the most ingenious generative models.
They aim to model reversing a Markov chain of the diffusion process illustrated in~\autoref{illustration_diffusion}. 
During training, noisy samples are obtained by incrementally adding noise to raw samples. The DDPM model then progressively reverses the diffusion process by predicting noise and denoising the samples. 
The loss is computed as the difference between the predicted noise and the Gaussian noise added during the diffusion process. 
In the inference stage, given a well-trained DDPM, it can generate realistic motions from a Gaussian distribution via the reversed diffusion process.

\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{figs/Visio-illustration_diffusion_re.pdf}
 \caption{Diffusion process and reversed process in DDPM. %\zhiming{typos in the figure: Gaussian Noise $->$ Gaussian noise, denosising $->$ denoising}
 }
 \label{illustration_diffusion}
\end{figure}

Owing to their power of generating realistic and high-quality samples, diffusion models have been applied in image/video generation\cite{rombach2022high,ho2022video}, anomaly detection\cite{wyatt2022anoddpm}, objection detection\cite{chen2022diffusiondet}, 3D reconstruction\cite{xu2022dream3d}, time series forecasting\cite{rasul2021autoregressive} and imputation\cite{tashiro2021csdi}. 
%\zhiming{Why do you break these into two paragraphs?}
%In a similar context\zhiming{Why do you treat images/time series differently? You can just say Diffusion has been successfully applied to many specific tasks and then focus on the HMP task.}, diffusion models have been used in time-series forecasting and imputation, which have also shown state-of-the-art performance. 
In a similar context, Tevet et al.\cite{tevet2022human} proposed a text-driven human motion synthesis method with diffusion models. 
Recently, Barquero et al. \cite{barquero2022belfusion} utilised a latent diffusion model to sample the diverse behaviour code to predict stochastic motions. 
Chen et al.\cite{chen2023humanmac} presented an end-to-end motion prediction framework based on diffusion models without complicated loss constraints and training processes. 
%Their work has demonstrated competitive performance in this domain.
%Current works BeLFusion \cite{barquero2022belfusion} and HumanMAC\cite{chen2023humanmac} have tried to forecast future human motions via diffusion model in latent and Discrete Cosine Transform (DCT) \cite{mao2019learning} space respectively. 
%\zhiming{Briefly introduce these two methods first and then point out their limitations and then your novelty. Currently, it is not clear how these two methods differ.}
However, existing methods usually produce unrealistic predictions, probably because they only focus on past human poses and neglect important information from other modalities.
%Although these diffusion-based methods have made significant contributions to stochastic HMP, unrealistic results can be yielded by only focusing on past human poses and neglecting important information from other modalities. 
To address this limitation, our method injects gaze-motion features into the denoising step through a cross-modal attention mechanism to generate more reasonable motion predictions.
%, which is used to capture the correlations between historical gaze-motion features and future motions and makes predictions better align with observed human behaviour.

%To address these problems, our gaze-guided diffusion model takes into account the coordination between gaze and human movements. By incorporating gaze information, we aim to generate more reasonable and plausible human motion predictions. This integration of gaze and human movement data allows for a more holistic understanding of human behaviour, resulting in improved motion synthesis that better aligns with intentions.
%\zhiming{Here we should explain the difference between our diffusion model and prior diffusion models}

%it is crucial to design a new diffusion-based HMP model that can forecast based on all informative modalities. 
%Inspired by the text-driven motion synthesis diffusion model\cite{zhang2022motiondiffuse}, the gaze-motion fused feature as a condition is added to the noise prediction network of the proposed model via a cross-attention mechanism in this paper. Meanwhile, following HumanMac\cite{chen2023humanmac}, the observed pose and gaze sequence is also added to the noise prediction network for the feature from the original scale. Through the above multi-scale "hints", the generation of prediction could be more controllable and accurate. 
%\zhiming{This is too detailed. Just say current diffusion models for HMP only used observed motions, while you used eye gaze and motions. Emphasise the key difference/novelty.}

==> zkmhtsrhjhszcdsvwdzpzpvnpcxyxrcp/sections/user_study.tex <==
\section{User Study}
%\zhiming{mention that this study is approved by the University.}
%Realism or trustworthiness can be subjective, so it would be hard to evaluate by numerical metrics\zhiming{No, this implies your numerical results are meaningless.}. 
%The quantitative and qualitative results 
%For example, the predictions of many failure cases can result in a very high APD value\cite{chen2023humanmac}. 
%To , we conducted an online user study to assess the realism of predicted motions.
To perform a comprehensive evaluation of the perceived precision and realism of the generated samples, we conducted a user study to assess model performance based on human perception and intuition. Participants were tasked with random samples predicted by different motion forecasting models. By collecting subjective rankings directly from individuals, the user study provided an intuitive approach to evaluate the aspects of the predictions that are challenging to assess objectively, such as naturalness, continuity, and the overall plausibility of the motions.% to a human observer.

\subsection{Assessment Details}
We randomly selected 4 sequences from the MoGaze dataset and 12 sequences from the GIMO dataset.
The difference in the number of selections between the two datasets can be attributed to the difference in the variety of actions included. While the MoGaze dataset consists of only two actions, the GIMO dataset contains a larger number of different actions. We compared our method with the best baseline HumanMAC. \textcolor{black}{The compared conditions were randomly provided to the users in order to avoid any potential bias.} Each method generated 10 predictions from random noise. \textcolor{black}{We set the sample size to 10 for a trade-off between the predictions’ diversity and users’ burden}. The participants in our study were then instructed to rank these predictions based on the following two key aspects:

\begin{itemize}
\item \textbf{Realism}: If these poses are physically plausible. You can check if there are any angle distortions, too short/long limbs, implausible poses, or any sudden or unreasonable changes during the whole motion.

\item \textbf{Precision}: If these motions align with the ground truth. You can measure the similarity between each motion and the ground truth.
\end{itemize}

The questionnaire utilised in our study was created using the \textit{Jotform} platform
%\footnote{·https://www.jotform.com/}.
The interface of our user study can be found in the supplementary material. A total of 21 individuals (11 males and 10 females, aged between 21
and 39 years, Mean= 26.3, SD=4.4) were recruited to take part in our user study via university mailing lists and social networks.
%\zhiming{add age and gender distribution} 
%participated in our user study. 
This user study is approved by the university.

\subsection{Evaluation}

As shown in \autoref{tab: user study}, our method outperforms HumanMAC in terms of both precision and realism. 74.6\% of the total responses considered predictions of our method as more precise while only 25.4\% regarded HumanMAC's results as more precise. From the perspective of realism, 67.7\% of the total responses considered the motions generated by our method as more realistic than HumanMAC
%showed that participants thought predicted motions from the proposed method with better realism.
%
%\zhiming{add statistical analysis} 
while only 33.3\% of the responses considered HumanMAC were able to generate more realistic predictions. 
To further validate our findings, we conducted a paired Wilcoxon signed-rank test, which revealed a statistically significant difference ($p<0.01$) between our method and HumanMAC in terms of both precision and realism.
%average ``more realistic selection’' from all responses. 
%Likewise, a statistically significant difference ($p<0.01$) between our method and HumanMAC in terms of average ``more precise selection’' from all responses.
%, achieving the highest average ranking of 1.691. This indicates that our method was perceived as the most realistic by the participants overall. 
%Remarkably, our method received the highest percentage of first-place rankings, with 49.52\%, indicating that it was consistently ranked as the most realistic option. Additionally, it obtained a respectable 31.88\% of second-place rankings. On the other hand, our method had the lowest percentage of third-place rankings at 18.60\%, suggesting that it was least frequently perceived as the least realistic option. In comparison, DLow obtained the highest percentage of second-place rankings at 39.13\%, but its first-place percentage was lower, at 26.33\%. This reveals that DLow was less frequently considered the most realistic option but often ranked as the second most realistic. HumanMAC, on the other hand, had the highest percentage of third-place rankings at 46.60\%, indicating that it was frequently perceived as the least realistic prediction. Moreover, its first and second-place percentages were the lowest among the three methods.
%To further validate our findings, we conducted a paired Wilcoxon signed-rank test, which revealed a statistically significant difference ($p<0.01$) between our method and the second-best method, DLow, in terms of average rankings from all responses.

\begin{table}[H]
  \caption{Results of the user study. Participants were required to measure the predictions from different methods according to precision and realism.}
  \label{tab: user study}
  \scriptsize%

	\centering%
  \begin{tabu}{%
	l%
	*{4}{c}%
	%
	}
  \toprule
    & More precise & More realistic   \\
  \midrule
   $HumanMAC$ & 25.4\% & 32.3\%\\
   $Ours$ &74.6\%&	67.7\%  \\

     
  
  \bottomrule
  \end{tabu}%
\end{table}
